Abstract Interpretation of Stateful Networks

Modern networks achieve robustness and scalability by maintaining states on their nodes. These nodes are referred to as middleboxes and are essential for network functionality. However, the presence of middleboxes drastically complicates the task of network verification. Previous work showed that the problem is undecidable in general and EXPSPACE-complete when abstracting away the order of packet arrival. We describe a new algorithm for conservatively checking isolation properties of stateful networks. The asymptotic complexity of the algorithm is polynomial in the size of the network, albeit being exponential in the maximal number of queries of the local state that a middlebox can do, which is often small. Our algorithm is sound, i.e., it can never miss a violation of safety but may fail to verify some properties. The algorithm performs on-the fly abstract interpretation by (1) abstracting away the order of packet processing and the number of times each packet arrives, (2) abstracting away correlations between states of different middleboxes and channel contents, and (3) representing middlebox states by their effect on each packet separately, rather than taking into account the entire state space. We show that the abstractions do not lose precision when middleboxes may reset in any state. This is encouraging since many real middleboxes reset, e.g., after some session timeout is reached or due to hardware failure.

==> absint.tex <==
\section{Abstract Interpretation Background}
\label{sec:absint-bg}

\subsection{Basic Concepts}
In this paper, a \emph{semantic domain}, or simply \emph{domain},
is a join-semilattice $D=(V_D, \aleq_D, \join_D, \bot_D)$.
%
We use semantic domains to represent the states of middleboxes
and the contents of channels (either concretely or abstractly).
We represent the set of (concrete and abstract) network configurations by applying standard domain constructors.

An abstract interpretation relative to a concrete domain $C$,
can be obtained by defining an abstract domain $A$ along with
an abstraction function $\alpha_{C,A} : V_C \rightarrow V_A$,
and a concretization function $\gamma_{A,C} : V_A \rightarrow V_C$.
We require the two functions to be monotone with respect to the
partial orders defined for $C$ and $A$, and to form a \emph{Galois connection},
denoted $(C, \gamma_{A,C}, \alpha_{C,A}, A)$:
\[
\begin{array}{ll}
(i) & \forall x\in V_C\;.\;x \aleq_C \gamma_{A,C}(\alpha_{C,A}(x)),\\
(ii) & \forall y\in V_A\;.\;\alpha_{C,A}(\gamma_{A,C}(y)) \aleq_A y \enspace.
\end{array}
\]

When the elements of the concrete domain, $V_C$, are sets,
the abstraction function can be
defined via the single-element abstraction function
$\beta_{C,A}(v)=\alpha_{C,A}(\{v\})$
and the concretization function can be defined via
abstraction:
\[
\begin{array}{rcl}
\alpha_{C,A}(c) &=& \bigsqcup\limits_{v \in c} \beta_{C,A}(v)\\
\gamma_{A,C}(a) &=& \bigsqcup \{c \in V_C \;|\; \alpha_{C,A}(c)\aleq_A a\}\enspace.
\end{array}
\]
%
In the sequel, we therefore define abstractions by only defining
the domains $C$ and $A$ and the single-element abstraction function $\beta$.

The semantics of a system can be defined relative to a domain $L$,
a monotone transformer $\Tr_L : V_L \rightarrow V_L$,
and an initial element $\Initial \in V_L$ as
$\lfp(\Tr_L)(\Initial_L)$.

For each monotone transformer $\Tr_C : V_C \rightarrow V_C$, a Galois connection $(C, \gamma_{A,C}, \alpha_{C,A}, A)$ induces the most precise transformer (also known as the \emph{best transformer})
$\Tr_A : V_A \rightarrow V_A$, defined as follows:
\[
\Tr_A(a) = \alpha_{A,C}(\Tr(\gamma_{A,C}(a)))\enspace.
\]

Unfortunately, when $V_C$ is infinite, this formulation does not result in an algorithm.

%Therefore, abstract interpretations often overapproximate
%the best transformer by a
%sound (and computable) transformer $\Tr_A^{\#}$ such that
%$\alpha(\Tr_C(x)) \aleq_A \Tr_A^{\#}(\alpha(x))$ holds.
%
An abstract interpretation can then be defined as
%relative to  a Galois connection $(C, \gamma, \alpha, A)$
%and a sound abstract transformer, as
$\lfp(\Tr_A)(\Initial_A)$ where $\Initial_A=\alpha_{A,C}(\Initial_C)$.

We say that an abstract domain $A$ is \emph{fixpoint-complete} relative to
another domain $C$, when the following holds:
\[
\alpha_{A,C}(\lfp(\Tr_C)(\Initial_C)) = \lfp(\Tr_A)(\Initial_A)\enspace.
\]

%\para{Abstract Interpretations as Non-standard Semantics.}
%The following definition provides a way to view the abstract interpretation without
%considering the representation of the abstract elements.

%\begin{definition}[Upper Closure Operator]
%\label{def:induced}
%Let a concrete semantics be defined by
%a semantic domain $C$, an initial element $\Initial_C$,
%and a transformer $\Tr_C$.
%%
%Further, let $(C,\gamma,\alpha,A)$ be a Galois connection.
%
%The induced \emph{upper closure operator} $\rho : C \rightarrow C$
%is defined as $\rho(c)=\gamma(\alpha(c))$.
%%
%The induced non-standard semantics is given by
%the domain whose elements are defined as $\{\rho(c) \;|\; c \in C\}$,
%the initial element $\rho(\Initial_C)$, and the transformer
%$\Tr_{\rho} = \rho \circ \Tr_C$.
%%with the partial order $c_1 \sqsubseteq c_2$ iff $\rho(c_1) \sqsubseteq_C \rho(c_2)$,
%%with the join operator defined as $$
%\end{definition}

\subsection{Systematic Domain Construction}
We now define domain constructors, which take sets
and create semantic domains, or take existing semantic domains
and create new semantic domains. The latter form of construction
also induces a Galois connection.

For a set of elements $V$, we define the corresponding \emph{flat domain} by adding the special values
$\bot$ and $\top$:
\[
\begin{array}{rcl}
\Flat(V) &\eqdef& (V \cup \{\bot,\top\}, \aleq, \join, \bot)\\
\aleq    &\eqdef& \{ (\bot,v) \;|\; v\in V\} \cup \{ (v,\top) \;|\; v\in V\} \enspace.
\end{array}
\]
The operator $\join$ is defined as the least upper bound (LUB) of a (possibly infinite) subset of $V \cup \{\bot,\top\}$.

This construction induces the Galois connection $(C,\gamma,\alpha,\Flat(V))$,
defined by the abstraction function
\[
\beta(c) = \left\{
                                                  \begin{array}{ll}
                                                    c, & c \in V\hbox{;} \\
                                                    \top, & \hbox{else.}
                                                  \end{array}
                                                \right.\enspace.
\]

\subsubsection{Disjunctive Completion Constructor}
We also define the corresponding \emph{powerset lattice} as follows:
\[
\PowLattice(V) \eqdef (\pow{V}, \subseteq, \cup, \emptyset) \enspace.
\]

Given a Galois connection $(C, \gamma, \alpha, A)$ with a most precise transformer $\Tr_A$,
we can define the more precise Galois connection $(C, \gamma, \alpha, L)$
as follows:
\[
\begin{array}{rcl}
L&=&\PowLattice(V_A)\\
\beta_{C,L}(c)&=&\{ \beta_{C,A}(c) \}\\
\gamma_{L,C}(\textit{xl})&=& \bigcup\limits_{a \in \textit{xl}}\gamma_{L,C}(a) \enspace.
\end{array}
\]
This construction, which we denote as $L=\pow{A}$, is called \emph{disjunctive completion}.

The most precise transformer for the disjunctive completion of $A$ can be computed as
\[
\Tr_{L}(\textit{xl}) = \{ \Tr_A(a) \;|\; a \in \textit{xl} \} \enspace.
\]

\subsubsection{Product Constructor}
Given two domains $A$ and $B$, we may combine
them to form the product domain $L_1 \times L_2$, defined
as $(V_A \times V_B, \aleq_{A\times B}, \join_{A\times B},
(\bot_A,\bot_B))$ where
$(v_1,v_2) \aleq_{A\times B} (v_1',v_2')$ if and only if $v_1 \aleq_A v_1'$
and $v_2 \aleq_B v_2'$ and $\join_{A\times B}$ is
defined point-wise on the corresponding components.
%
From the Galois connections $(C, \gamma_{C,A}, \alpha_{A,C}, A)$ and
$(C, \gamma_{C,B}, \alpha_{B,C}, B)$ defined by the corresponding
abstraction functions $\beta_{A\times B} : V_C \rightarrow V_{A}$
and $\beta_{A\times B} : V_C \rightarrow V_{B}$, we can obtain the Galois connection
$(C, \gamma_{A\times B}, \alpha_{A\times B}, A \times B)$ via the
abstraction function $\beta_{A\times B}(x) = (\beta_A(x), \beta_B(x))$.

Unfortunately, the most precise transformer for a product domain does not generally have a computable formulation.
%
Instead, we define the sound \emph{independent attribute} transformer:
\[
\Tr_{A\times B}(a,b) = (\Tr_A(a), \Tr_B(b)) \enspace.
\]

%We may also combine them by first taking their product and then applying
%disjunctive completion, which we refer to as their \emph{relational product}: $\pow{L_1 \times L_2}$.

\subsubsection{Function Space Constructor}
Given a finite set $S$, we can lift a domain
$L=(V_L,\aleq,\join,\bot)$ to the space of functions
from $S$ to $L$ by forming the domain
$S \rightarrow L \eqdef (S \rightarrow V_L,\aleq_{S\rightarrow L},\join_{S\rightarrow L},\lambda s\,.\,\bot)$
where $f_1 \aleq_{S\rightarrow L} f_2$ if and only if $\forall s \in S\,.\,f_1(s) \aleq f_2(s)$, and
$f_1 \join_{S\rightarrow L} f_2 \eqdef \lambda s\,.\, f_1(s)\join f_2(s)$.
%
Given a Galois connection $(C,\gamma,\alpha,L)$,
this construction induces the Galois connection of the space of functions $(C,\gamma_{S\rightarrow L},\alpha_{S\rightarrow L},S\rightarrow L)$
defined by the abstraction function
$\alpha_{S\rightarrow L}(f) = \lambda s\,.\, \alpha(f(s))$.

Similar to the product constructor, the most precise transformer does not have a general computable formulation.
%
We define the \emph{independent attribute} sound transformer as follows:
\[
\Tr_{S\rightarrow L}(f) = \lambda s\,.\, \Tr_L(f(s)) \enspace.
\]

\newcommand{\XF}{\textit{XF}}

\begin{theorem}[Completeness for Local Distributive Transformers]
Let $L=(V_L,\aleq,\join,\bot)$ be a domain and let $S$ be a finite set
such that $\Tr : (S\rightarrow V_L) \rightarrow (S\rightarrow V_L)$
is a transformer for $S\rightarrow L$.
%
Further, let $\Tr_1[s] : V_L \rightarrow V_L$
be a \emph{sub transformer} such that the following holds:
\begin{equation}
\label{LocalSubTransformer}
\forall s \in S \;.\; \Tr(f)(s) = \Tr_1[s](f(s))
\end{equation}
and the sub transformer is distributive:
\begin{equation}
\label{DistributiveSubTransformer}
\forall s \in S \;.\; \forall X \in 2^{V_L} \;.\; \Tr_1[s](\join_L X) = \join_L \{ \Tr_1[s](l) \;|\; l \in X\}\enspace.
\end{equation}

We define the \emph{local transformer} $\Tr_1 : (S\rightarrow V_L) \rightarrow (S\rightarrow V_L)$ as follows:
\[
\Tr_1(f) = \lambda s\in S\;.\; \Tr_1[s](f(s)) \enspace.
\]
Then, (1) the identity $\Tr(f) = \Tr_1(f)$ holds and
(2) for every set of functions $\XF \in 2^{S\rightarrow L}$, we have that
the following holds:
\[
\join_{S\rightarrow L} \{\Tr(f) \;|\; f\in\XF\} = \Tr_1(\join_{S\rightarrow L} \XF) \enspace.
\]
\end{theorem}
\begin{proof}
The first claim follows directly from \ref{LocalSubTransformer}.
The second claim can be proved as follows:
\[
\begin{array}{l}
\join_{S\rightarrow L} \{\Tr(f) \;|\; f\in\XF\} = \\
\lambda s\in S \;.\; \join_L \{ \Tr(f)(s) \;|\; f\in\XF\} =\\
\lambda s\in S \;.\; \join_L \{ \Tr_1(f)(s) \;|\; f\in\XF\} =\\
\lambda s\in S \;.\; \join_L \{ \Tr_1[s](f(s)) \;|\; f\in\XF\} =\\
\lambda s\in S \;.\; \Tr_1[s](\join_L \{ f(s) \;|\; f\in\XF\}) =\\
(\text{From }\ref{DistributiveSubTransformer})\\
\lambda s\in S \;.\; \Tr_1[s](\, (\lambda s'\;.\;\join_L\{f(s') \;|\; f\in \XF\})(s)\,)=\\
\Tr_1(\lambda s\in S \;.\;\join_L\{f(s) \;|\; f\in \XF\}) =\\
\Tr_1(\join_{S\rightarrow L} \XF) \enspace.
\end{array}
\]
\end{proof}

\TODO{Explain partial concretization. }

\newcommand{\expand}{\textit{expand}}
The theorem above can be combined with the notion of partial concretization as follows.
Let $L=(V_L,\aleq,\join,\bot)$ be a domain and let $S$ be a finite set.
Then, elements of $S\rightarrow L$ can be partially concretized to the elements
of $(S\times S)\rightarrow (L\times L)$ via the function
$\expand(f) = \lambda s_1,s_2\in S \;.\; (f(s_1),f(s_2))$.
%
Now, if $\Tr_2[s,s'] : (L\times L)) \rightarrow (L\times L)$
is a local distributive transformer for the expanded domain, then
the transformer
\[
\lambda s\;.\; \join_L \{ first(\Tr_2[s,s'](\expand(f)(s,s'))) \;|\; s' \in S \}
\]
is $\alpha$-complete for $S\rightarrow L$.

\para{A Note on Notations.}
In the paper, we will slightly abuse notation by using a set of
values to denote the corresponding flat domain and using product,
functions, and powersets to stand for the corresponding domain
constructors. 

==> abstractions-old.tex <==



%\section{Equivalent Semantics based on Packet Space}

\section{Abstract Interpretation of Stateful Networks}

In this section we define an abstract interpretation of stateful networks, obtained by a sequence of sound abstractions. The first two abstractions correspond to the relaxations of the semantics described in \Cref{sec:network-semantics}. The third abstraction is a cartesian abstraction. Interestingly, for unordered reverting networks the cartesian abstraction is complete. Namely, it does not lead to any additional precision loss.

\TODO{this section is not consistent with description as functions. In addition, here $\sigma$ stands for the entire state, as opposed to $(\sigma,C)$ before}

\subsection{Concrete Domain}
\TODO{present it as a relational product domain. Then we can define abstractions of middlebox state and abstractions of channel state independently and combine them either via relational product or via cartesian product}
Recall that the set of concrete unordered configurations is defined as $\Sigma^u = (M\to \Sigma^r[M])\times(E \to \mset{P})$.
%
To facilitate the abstractions employed in this work, we use a vector representation which allows us to abstract the middlebox states and the channel states separately, and combine these abstraction either by a relational product construction, which maintains correlations, or by a cartesian product construction.
%
%To simplify the presentation, we will use a vector representation.
Let $m_1,\ldots,m_\ell$ be an enumeration of $M$ and $e_1,\ldots,e_k$ be an enumeration of $E$.
%
Recall that $\Sigma^r[m]$ denotes the set of middlebox states of $m\in M$.
Let $\Sigma^r[e] : \mset{P}$ denote the set of states (i.e., content)
of a channel $e$.
%
Unordered configurations can be therefore represented by the set of vectors
$\Sigma^r[m_1]\times\ldots\times\Sigma^r[m_{\ell}]\times \Sigma^r[e_1]\times\ldots\times \Sigma^r[e_k]$.
%
The state space of the network is therefore $\pset(\Sigma^r[m_1]\times\ldots\times\Sigma^r[m_{\ell}]\times \Sigma^r[e_1]\times\ldots\times \Sigma^r[e_k])$. An explicit search for a state violating the safety property would be exponential in the state space (and thus doubly-exponential in the number of hosts in the network).


\subsection{Unordered Channels Abstraction}
\label{sec:unordered-semantics}

We first define an abstraction of the network that captures the unordered overapproximation of the network semantics.
%, where channels do not necessarily preserve the packet transmission order. Namely, packets in the same channel may be processed in a different order than the order in which they were received.

%Recall that the set of unordered configurations is denoted $\UnConfs$. We now define an abstract domain  Galois connection between $\powerset{\ConcConfs}$ and $\powerset{\UnConfs}$, where the abstraction maps ordered channels to their multiset counterpart.

\para{Unordered Network Configurations}
The set of  \emph{Unordered configurations}, defined next, is denoted $\Sigma^u$.
An \emph{unordered network configuration} $\sigma^u \in \Sigma^u = (M\to \Sigma^r[M])\times(E \to \mset{P})$
assigns communication channels to multisets of packets, thus abstracting away the order
between packets.
%
%The set of all \emph{Unordered configurations} is denoted $\Sigma^u$.

This allows us to define the Unordered abstraction of network states
$\beta^u : \Sigma^o \rightarrow \Sigma^u$
\[
\begin{array}{ll}
\beta^u(\sigma[m_1],\ldots,\sigma[m_\ell],\sigma[e_1],\ldots,\sigma[e_k]) =\\
\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;(\sigma[m_1],\ldots,\sigma[m_\ell],\toMultiset{\sigma[e_1]},\ldots,\toMultiset{\sigma[e_k]})
\end{array}
\]
which is lifted to a Galois connection between $(\powerset{\Sigma^o}, \subseteq)$ and $(\powerset{\Sigma^u}, \subseteq)$, where the abstraction maps ordered channels to their multiset counterpart.
Formally, $\alpha^u(\omega^o) = \{ \beta^u(\sigma^o) \mid \sigma^o \in \omega^o \}$, and
$\gamma^u(\omega^u) = \{ \sigma \in \Sigma^o \;|\; \beta^u(\sigma) \in \omega^u\}$.

%and the partial order $\omega \sqsubseteq^u \omega'$ iff  \TODO{complete and fix. probably need join as well}
%This allows us to define the concretization function $\gamma^c : \Sigma^c \rightarrow \Sigma^s$ as
%$\gamma^c(\omega) = \{ \sigma \in \Sigma^s \;|\; \beta(\sigma) \sqsubseteq^c \omega\}$.


\para{Abstract Transformer}
We denote the corresponding best abstract transformer by \TODO{complete}.
\TODO{do we want to include the explicit transformer?}

\ignore{
\TODO{revise to describe the transformer}
the unordered semantics of a transition in the network as $(\sigma,C) \xrightarrow{p,e,m}_u (\sigma',C')$ where
the following hold:
(i) $p$ is some packet on the channel $e \in E$,
(ii) the channel $e$ is an ingress channel of middlebox $m$,
(iii) there exists a command $c$ in middlebox $m$ s.t. $\sembr{c}_{pre}$ holds in state $\sigma(m)$ for packet $p$,
(iv) the safety condition $\msafe{m}$ of the middlebox $m$ holds for the middlebox state $\sigma(m)$ for packet $p$,
(v) $C'$ is the result of removing packet $p$ from the multiset assigned to channel $e$ and adding the result of $\sembr{c}_{out}$ to the the appropriate channels via multiset sum, and
(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.

\TODO{perhaps just remove the above? Why is it helpful? }
}

\TODO{state completeness of the least fixpoint computation? }


\subsection{Sticky Channels Abstraction}

The next abstraction that we consider is based on the reverting network semantics, and exploits its sticky properties.
%In case that the middleboxes are indeed reverting, this is not an abstraction.


\para{Sticky Channels Network Configurations}

When a network has the sticky packets property, it is no longer necessary to maintain the cardinality of every packet type on every channel. Instead, it is sufficient to record whether a packet arrived on the channel at some point.
%
We can then define the \emph{sticky channel configuration} of a network as $\sigma^s \in \Sigma^s = (M\to \Sigma^r[M])\times(E \to 2^P)$, which assigns communication channels to sets of packets, abstracting away the cardinality of each packet.
%
The set of all \emph{Sticky configurations} is denoted $\Sigma^s$. %\TODO{complete}

This allows us to define the Sticky abstraction of network states
$\beta^s : \Sigma^u \rightarrow \Sigma^s$
\[
\begin{array}{ll}
\beta^s(\sigma[m_1],\ldots,\sigma[m_\ell],\sigma[e_1],\ldots,\sigma[e_k]) =\\
\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\;(\sigma[m_1],\ldots,\sigma[m_\ell],\toSet{\sigma[e_1]},\ldots,\toSet{\sigma[e_k]}).
\end{array}
\]
We define  a Galois connection between $(\powerset{\Sigma^u}, \subseteq)$ and $(\powerset{\Sigma^s}, \subseteq$, where the abstraction maps unordered (multiset) channels to their sticky (set) counterpart.
Formally, $\alpha^s(\omega^u) = \{ \beta^s(\sigma^u) \mid \sigma^u \in \omega^u \}$, and
$\gamma^s(\omega^s) = \{ \sigma \in \Sigma^u \;|\; \beta^s(\sigma) \in \omega^s\}$.


%and the partial order $\sigma \sqsubseteq^s \sigma'$ iff for every $\mboxe \in \mboxes$, $\sigma[m] = \sigma'[m]$ and for every $e \in E$, $\sigma[e] \subseteq \sigma'[e]$.
%We lift this partial order to sets of sticky configurations in the natural way: $\omega \sqsubseteq^s \omega'$ iff for every $\sigma \in \omega$ there exists $\sigma' \in \omega'$ such that $\sigma \sqsubseteq^s \sigma'$.
%This induces a join operator $\sqcup^s : \powerset{\Sigma^s} \times \powerset{\Sigma^s} \rightarrow \powerset{\Sigma^s}$ where $ \omega \sqcup^s \omega' = $ \TODO{complete and verify. }.
%
%\TODO{we have two options to define this abstract domain: either with set inclusion and set union as partial order and join, or as defined above. Which one is better?}
%
%We now define  a Galois connection between $(\powerset{\Sigma^u}, \subseteq)$ and $(\powerset{\Sigma^s}, \sqsubseteq^s)$, where the abstraction maps unordered (multiset) channels to their sticky (set) counterpart.
%Formally, $\alpha^s(\omega^u) = \bigsqcup^s_{\sigma^u \in \omega^u} \{ \beta^u(\sigma^o)\} $, and
%$\gamma^s(\omega^s) = \{ \sigma \in \Sigma^s \;|\; \{\beta^s(\sigma)\} \sqsubseteq^s \omega^s\}$.


\para{Abstract Transformer}
We denote the corresponding best abstract transformer by \TODO{complete}.
\TODO{do we want to include the explicit transformer?}

\ignore{
\TODO{revise to describe the transformer}
\para{Sticky Channels Network Transitions}
We define the sticky Channels semantics of a transition in the network as $(\sigma,C) \xrightarrow{p,e,m}_s (\sigma',C')$ where
the following hold:
(i) $p$ is some packet on the channel $e \in E$,
(ii) the channel $e$ is an ingress channel of middlebox $m$,
(iii) there exists a command $c$ in middlebox $m$ s.t. $\sembr{c}_{pre}$ holds in state $\sigma(m)$ for packet $p$,
(iv) the safety condition $\msafe{m}$ of the middlebox $m$ holds for the middlebox state $\sigma(m)$ for packet $p$,
(v) $C'$ is the result of adding the result of $\sembr{c}_{out}$ to the appropriate channels via set union, and
(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.

\TODO{perhaps just remove the above? Why is it helpful? }
}

\TODO{state completeness of the least fixpoint computation? }


==> abstractions.tex <==
\section{Abstract Interpretation of Stateful Networks}
\label{sec:absint}

\newcommand{\NetFIFO}{\textit{NFIFO}}
\newcommand{\RvtUnordDom}{\textit{NRU}}
\newcommand{\Cart}{\textit{NCart}}
%\newcommand{\PFIFO}{\textit{PFIFO}}
%\newcommand{\PMSet}{\textit{PMSet}}
%\newcommand{\PSet}{\textit{PSet}}
%\newcommand{\Rvt}{\textit{Rvt}}
%\newcommand{\MB}{\textit{MB}}
\newcommand{\PFIFO}{\packets^{*}}
\newcommand{\PMSet}{(\packets\rightarrow\Nat)}
\newcommand{\PSet}{\pow{\packets}}
\newcommand{\Rvt}{\MB}
\newcommand{\MB}{\Sigma[M]}
\newcommand{\ms}{\textit{ms}}

\begin{figure}
  \centering
  \includegraphics[width=0.47\textwidth]{img/AbstractionsHierarchy}
  \caption{A hierarchy of network abstract domains. Dashed edges represent sound but incomplete abstractions,
  and solid edges represent complete abstractions.}
  \label{fig:abstractions-hierarchy}
\end{figure}

In this section, we define a hierarchy of abstractions,
which is shown in \Cref{fig:abstractions-hierarchy},
over the concrete network semantics defined in \secref{network-semantics}.
%
The abstractions apply either to the channel contents,
to the middlebox states,
or to the correlations between these individual components.

We assume the reader is familiar with the theory of abstract
interpretation~\cite{cousot1979systematic,PrinciplesOfPA},
and defer the definition of \emph{semantic domains},
\emph{Galois connection},
\emph{best transformer},
and domain constructors to \appref{absint-bg}.

For each point in the hierarchy, we define the abstract domain,
the abstraction function, and a \emph{non-standard semantics}
in terms of the transition relation between network configuration
induced by the abstraction.

\begin{definition}[Abstraction-induced Transition Relation]
\label{def:inducedTR}
Let $(\pow{\Sigma^o}, \gamma, \alpha, A)$ be a Galois connection
between the set of network configurations and the elements of
an abstract domain $A$.
%
The induced transition relation is defined as
%The transition relation induced by the Galois connection is
%defined as
\[
\begin{array}{l}
c_1 \rightarrow^A C_2 \text{ if and only if }\\
\exists c_1' \in \gamma(\alpha(c_1)), c_2' \in \gamma(\alpha(c_2))\;:\;
c_1' \rightarrow^o c_2'
\end{array}
\]
where $c_1,c_2,c_1',c_2' \in \Sigma^o$.
\end{definition}


%We start with a primer on abstract interpretation and then use
%the definitions to formally define the points in the abstraction %hierarchy.
%
%For each point, \TODO{not for each point: do we have a semantics for the cartesian domain?}
%we explain how to view it intuitively as
%a non-standard network semantics and state the complexity of soundly
%verifying network safety.
%For the key points,
%we explain how to view them as
%non-standard network semantics. Each non-standard semantics defines %transitions over the \emph{concrete} network configurations that are %induced by the corresponding abstract domain.
%Finally, we state the complexity of soundly
%verifying network safety and discuss completeness.

\subsection{A Hierarchy of Abstract Domains for Stateful Networks}

The set of concrete network configurations defined in \secref{network-semantics} can be seen from the perspective of systematic domain construction.

\begin{definition}[Ordered Network Domain]
The ordered network domain is obtained by
(i) taking the flat lattice of channel contents for
each channel,
(ii) using the set of middlebox states $\Sigma[m]$ to construct
the flat lattice of middlebox states,
and finally
(iii) combining them via function and relational domain constructors:
\[
\begin{array}{rcl}
%\PFIFO      &\eqdef& \Flat(\packets^{*})\\
%\MB         &\eqdef& \Flat(\Sigma[m])\\
\NetFIFO    &\eqdef& \pow{M\rightarrow \MB \times E\rightarrow \PFIFO}
\enspace.
\end{array}
\]
\end{definition}

We apply abstractions to different components of this construction
to obtain different abstract interpretations.

\begin{definition}[Abstract Error States]
Let $(\NetFIFO,\gamma,\alpha,A)$ be a Galois connection for
a network abstract domain $A$.
We say that an abstract state $a \in V(A)$
is an \emph{abstract error state} if $\gamma(a)$ contains an error configuration.
\end{definition}

\begin{definition}[Abstract Safety Verification]
The abstract safety verification problem, relative to a network abstract domain $A$, is to decide whether
$\lfp(T_A)(\Initial_A)$ is an abstract error state.
\end{definition}

\subsection{Unordered Network Semantics}
\label{sec:unordered-semantics}

We first define an abstract domain that abstracts away the order on channels. This domain induces a semantics where channels do not necessarily preserve the packet transmission order. Namely, packets in the same channel may be processed in a different order than the order in which they were received.

\begin{definition}[Unordered Channel Domain]
The \emph{unordered channel domain} (for a single channel) is defined as
the flat lattice of multisets of packets:
$\packets\rightarrow \Nat$.
%
The corresponding abstraction function is defined as $\lambda p \;.\; \# p \in \overline{p}$,
where $\# p$ denotes the number of appearances of the packet $p$ in a sequence of packets $\overline{p}$.
\end{definition}

\begin{definition}[Unordered Network Domain]
The \emph{unordered network domain} is defined as
\[
\pow{M\rightarrow \MB \times E \rightarrow \PMSet} \enspace.
\]
\end{definition}

\ignore{
\para{Unordered Network Configurations}
\TODO{keep configurations the same. Move this to abstraction section}
An \emph{unordered network configuration} $\Sigma^u = (M\to \Sigma[M])\times(E \to \mset{\packets})$
assigns communication channels to multisets of packets, thus abstracting away the order
between packets.
%
The set of \emph{Unordered configurations} is defined as $\Sigma^u = $. \TODO{complete}

We denote the unordered initial state by $(\sigma_I,\lambda\,e\in E\,.\, \lambda\,p\in \packets\,.\, 0)$,
where $\sigma_I$ denotes the initial state of all middleboxes.
}

\ignore{
\TODO{revise to describe the transformer}
the unordered semantics of a transition in the network as $(\sigma,\pi) \xrightarrow{p,e,m}_u (\sigma',\pi')$ where
the following hold:
(i) $p$ is some packet on the channel $e \in E$,
(ii) the channel $e$ is an ingress channel of middlebox $m$,
(iii) there exists a command $c$ in middlebox $m$ s.t. $\sembr{c}_{pre}$ holds in state $\sigma(m)$ for packet $p$,
(iv) the safety condition $\msafe{m}$ of the middlebox $m$ holds for the middlebox state $\sigma(m)$ for packet $p$,
(v) $\pi'$ is the result of removing packet $p$ from the multiset assigned to channel $e$ and adding the result of $\sembr{c}_{out}$ to the the appropriate channels via multiset sum, and
(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.

\TODO{perhaps just remove the above? Why is it helpful? }
}

The unordered network domain induces the following non-standard network semantics:

\begin{lemma}[Induced Unordered Network Semantics]
The non-standard semantics over the concrete network configurations induced by the network domain
abstraction is given by the transitions
$(\sigma,\pi) \xrightarrow{p,e,m}_{u} (\sigma',\pi')$, where all conditions are as in the case of ordered transitions, with the exception of condition (i) that changes as follows:
(i) $p$ is \emph{some} packet on the channel $e \in E$. Namely, a transition can be triggered by \emph{any} packet on the ingress channel of a middlebox. Note that $(\sigma, \pi), (\sigma', \pi')$ are concrete configurations in  $\Sigma^o = (M\to \Sigma[M])\times(E \to \packets^{*})$.
%(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
%$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.
%In both cases, error transitions remain unchanged.
\end{lemma}

%\para{Unordered Network Transitions}
%%\TODO{say that this is the best transformer}
%The \emph{unordered semantics} of a transition in the network, induced by the unordered network domain is the following.
%For $(\sigma, \pi), (\sigma', \pi') \in \Sigma^o = (M\to \Sigma[M])\times(E \to \packets^{*})$, an unordered  transition $(\sigma,\pi) \xrightarrow{p,e,m}_u (\sigma',\pi')$ exists if the conditions of concrete (ordered) transitions hold, except that condition (i) changes to:
%(i) $p$ is \emph{some} packet on the channel $e \in E$. Namely, a transition can be triggered by \emph{any} packet on the ingress channel of a middlebox.
%%Error transitions are also adapted similarly.

\ignore{
We define the unordered semantics of a transition in the network as $(\sigma,C) \xrightarrow{p,e,m}_u (\sigma',pi')$ where
the following hold:
(i) $p$ is \emph{some} packet on the channel $e \in E$,
(ii) the channel $e$ is an ingress channel of middlebox $m$,
(iii) there exists a command $c$ in middlebox $m$ s.t. $\sembr{c}_{pre}$ holds in state $\sigma(m)$ for packet $p$,
(iv) the safety condition $\msafe{m}$ of the middlebox $m$ holds for the middlebox state $\sigma(m)$ for packet $p$,
(v) $C'$ is the result of removing packet $p$ from the multiset assigned to channel $e$ and adding the result of $\sembr{c}_{out}$ to the the appropriate channels via multiset sum, and
(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.
}

%The transformer, denoted $\Tr^u$, the collecting semantics, denoted %$\BB{\Net}^u$, as well as
%the safety verification problem for the unordered network semantics are %defined in the same way as in the ordered case.

\begin{theorem}
\label{thm:UnorderedUndecidable}
The safety verification problem for unordered network semantics
is EXPSACE-complete~\cite{velner2016some}.
\end{theorem}

\subsection{Reverting Network Semantics}
\label{sec:reverting-semantics}

\TODO{Explain why the abstract domain is (almost) the same as the concrete.}

The next abstract domain that we consider induces a semantics that allows middleboxes to revert to their initial state after every transition.
This semantics does not change the set of configurations, but increases the set of transitions to include reverting transitions.

\begin{definition}[Reverting Middlebox Domain]
The \emph{reverting middlebox domain} (for a single middlebox) is defined as $\Sigma[m]$.
The corresponding Galois connection is induced by the
following abstraction function over middlebox states:
$\lambda s \in \Sigma[m]\;.\; \{s,\sigma_I(m)\}$.
That is, a middlebox $m$ is considered to be simultaneously in a specific state $s$ and its initial state $\sigma_I(m)$.
\end{definition}

\begin{definition}[Reverting Network Domain]
The \emph{reverting network domain} is defined as
\[
\pow{M\rightarrow \Rvt \times E \rightarrow \PFIFO} \enspace.
\]
\end{definition}

The reverting network domain induces the following non-standard network semantics:

\begin{lemma}[Induced Reverting Network Semantics]
The non-standard semantics over the concrete network configurations induced by the reverting network domain
abstraction is given by the transitions
$(\sigma,\pi) \xrightarrow{p,e,m}_{or} (\sigma',\pi')$, where all conditions are as in the case of ordered transitions, with the exception of condition (iii) that changes as follows:
(iii) $\sigma(m) \xrightarrow{(p, e)/(p_1, e_2), \ldots, (p_k, e_k)} \sigma'(m)$ or $\sigma'(m) = \sigma_I(m)$, meaning that the middlebox $m$ reverts to its initial state.
%(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
%$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.
%In both cases, error transitions remain unchanged.
\end{lemma}

\begin{theorem}
\label{thm:RevertingUndecidable}
The safety verification problem for the reverting network semantics
is undecidable.
\end{theorem}

\subsection{Reverting Unordered Network Semantics}
\label{sec:sticky-semantics}

By combining the two abstractions defined above,
we obtain the next abstract domain and overapproximate semantics.

\begin{definition}[Reverting Unordered Network Domain]
The reverting unordered network domain is defined as:
\[
\RvtUnordDom \eqdef \pow{M\rightarrow \Rvt \times E \rightarrow \PMSet} \enspace.
\]
\end{definition}

\begin{lemma}[Induced Reverting Unordered Network Semantics]
The induced reverting unordered network semantics is given by taking
the union of transitions of the unordered network semantics
and the reverting semantics.
\end{lemma}

\begin{theorem}
\label{thm:reverting-unordered-conphard}
The safety problem for reverting unordered networks is coNP-hard.
\end{theorem}

The reverting unordered semantics is
not directly implementable (the set of packet multisets is infinite).
We continue by proving and utilizing properties of the semantics,
which allows us to apply further abstractions, while still maintaining
fixpoint-completeness, leading us to the
\emph{Cartesian network domain}.

\subsection{Utilizing Sticky Properties}

Unordered reverting networks have two useful properties that can help us reduce the complexity of searching for an error state, namely the \emph{sticky states} property and the \emph{sticky packets} property. Intuitively, the sticky properties state that if an event occurs in some run of the network, then any run has an extension in which that event occurs. Consequently, we can disregard the multiplicity of packets on the channels and the correlation between the state of a middlebox $m$ and the states of other middleboxes as well as the states of the channels that are not connected to the middlebox $m$.

The following lemma shows that the reverting unordered semantics
maintains the sticky packet property.

\begin{lemma}
\label{lem:sticky-packets}
For every channel $e$ and packet $p$:
If in some reachable configuration $e$ contains $p$, then every run can be extended such that $e$ will eventually contain $p$.

Moreover, every run can be extended such that $e$ will eventually contain $n$ copies of $p$ (for every $n>0$).
\end{lemma}

%\newcommand{\AppearsOn}[2]{{#1}\text{ on }{#2}}
%\begin{corollary}
%Consider the set of all abstract configurations denoting
%the fact that a packet $p$ may appear on channel $e$:
%\[
%X = \{(e,p) \;|\; (\sigma, \omega) \in \BB{N}^\RvtUnordDom \,,\,
%\omega(e)(p) > 0\} \enspace.
%\]
%
%Then the reverting unordered semantics is closed under ...
%\[
%\begin{array}{l}
%(e,p) \in X \land (\sigma, \omega) \in \BB{N}^\RvtUnordDom \implies\\
%\{ (\sigma, \omega') \;|\; \omega'(e)(p) = k, k >0\} \subseteq \BB{N}^\RvtUnordDom
%\end{array}
%\]
%\end{corollary}

When a network has the sticky packets property, it is no longer necessary to maintain the cardinality of every packet on every channel and it is not necessary to maintain the correlation between a channel and the set of packets
that can simultaneously appear there.
Instead, it is sufficient to record, for each individual channel $e$ and individual packet $p$,
whether $p$ has arrived on $p$ at some point. %We denote this fact by the predicate $\AppearsOn{p}{e}$.

We now show that unordered reverting networks have the sticky states property.

\begin{lemma}
\label{lem:sticky-states}
For every channel $e$, packet $p$, middlebox $m$ and state $\sigma_m$ of $m$:
If in some reachable configuration channel $e$ contains $p$ and in some (possibly other) reachable configuration $m$ is in state $\sigma_m$, then %every run can be extended such that eventually we get to 
there exists a reachable configuration where simultaneously $e$ contains $p$ and $m$ is in state $\sigma_m$.
%If in some scenario channel $c$ contains $p$ and $m$ is in state $q_m$, then every scenario can be extended such that eventually we get to a configuration where simultaneously $c$ contains $p$ and $m$ is in state $q_m$.
\end{lemma}

\ignore{
\TODO{revise to describe the transformer}
\para{Sticky Channels Network Transitions}
We define the sticky Channels semantics of a transition in the network as $(\sigma,\pi) \xrightarrow{p,e,m}_s (\sigma',\pi')$ where
the following hold:
(i) $p$ is some packet on the channel $e \in E$,
(ii) the channel $e$ is an ingress channel of middlebox $m$,
(iii) there exists a command $c$ in middlebox $m$ s.t. $\sembr{c}_{pre}$ holds in state $\sigma(m)$ for packet $p$,
(iv) the safety condition $\msafe{m}$ of the middlebox $m$ holds for the middlebox state $\sigma(m)$ for packet $p$,
(v) $C'$ is the result of adding the result of $\sembr{c}_{out}$ to the appropriate channels via set union, and
(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.

\TODO{perhaps just remove the above? Why is it helpful? }
}

\TODO{Explicitly write the final abstraction, transformer,
and complexity.} 

==> cartesian-semantics.tex <==
\subsection{Cartesian Network Abstraction}
\label{sec:cartesian-semantics}

Utilizing the properties of the reverting unordered semantics,
we obtain the following domain
\begin{definition}[Cartesian Network Domain]
The \emph{Cartesian network domain} is defined as:
\[
\Cart \eqdef M\rightarrow \pow{\MB} \times E \rightarrow \PSet \enspace.
%\times (\{ \AppearsOn{m}{\sigma(m)} \;|\; m \in M, \sigma \in \Sigma[m]\} \cup \{ \AppearsOn{p}{e} \;|\; e \in E, p \in \packets \})
\]
\end{definition}

The best transformer for the Cartesian network domain can be computed as follows:
\[
\begin{array}{rcl}
\Tr_{\Cart}(\eta,\kappa) &=& (\eta \cup \eta', \kappa \cup \kappa')\\
\eta' &=& \lambda m\;.\; \{s' \;|\; s\in \eta(m),\\
      & &  s \xrightarrow{(p, c)/\{(p_i, c_i)\}_{i=1..k}} s', p \in \kappa(c)\}\\
\kappa' &=& \{c_i\mapsto p_i \;|\; s\in \eta(m),\\
      & &  s \xrightarrow{(p, c)/\{(p_i, c_i)\}_{i=1..k}} s', p \in \kappa(c)\}\\
\end{array}
\]

\para{Complexity}
At each iteration of the fixed-point loop the algorithm either adds at least one new packet to a channel, or adds at least one new state to a middlebox.
In all, the algorithm is polynomial in the state space of the middleboxes of the network as well as in the state space of packets in the network.

However, the state space of the middleboxes of the network may be exponential in the number of hosts in the network, e.g. if one of the dimensions of a middlebox is $H$, then at worst we would have to store all subsets of $H$, leading to $2^{|H|}$ iterations of the fixed point algorithm.

The complexity is then $O(|H|^2|M|2^{|H|})$.

\begin{lemma}[Induced Cartesian Semantics]
The non-standard semantics induced by the network domain
abstraction is given by the transitions
$(\sigma,\pi) \xrightarrow{p,e,m}_{or} (\sigma',\pi')$, where all conditions are as in the case of
the reverting unordered transitions, with the exception that the state of the middlebox $m$ in $\sigma'$
may be any one of the states that it has taken in the past. \TODO{shouldn't there be something similar for the packets?}
%
That is, the semantics is history-oblivious with respect to middlebox states and the contents of
their incident channels.
\end{lemma}

%\para{Cartesian Network Transitions}
%We define the Cartesian semantics of a transition in the network as
%$\omega \xrightarrow{i}_u \omega'$
%where the following hold:

\lemref{sticky-states} implies the following theorem:
\begin{theorem}
The Cartesian abstraction is safe and complete for reverting middleboxes. i.e. if there exists a scenario violating safety under the Cartesian semantics then there exists a scenario violating safety under the sticky channel semantics and vice versa.
\end{theorem}

%\subsection{Computing the Abstract Least Fixed Point}

\TODO{talk about the locality of the computation of the best abstract transformer and how we actually do it}

\ignore{
\subsection{Computing the Least Fixed Point}
In this section, we present an algorithm that computes the least fixed point of a reverting network over the Cartesian abstraction presented in \secref{cartesian-abstraction}.

\begin{figure}[t]
\begin{tabbing}
m\=m\=m\=m\=m\=m\=m\=\kill
$\bforeach~ m\in M$ do \\
\> $\mathit{packetSeen}(m)$ := $\mathit{NeighborHostPackets}(m)$\\
\> \TODO{RM: why is this different from the empty set?}\\
\> $\mathit{reachableStates}(m)$ := $\mathit{InitialRelationValues}(m)$\\
$\bwhile$ fixed-point not reached \\
\> $\bforeach~ m\in M$ do \\
\>\> $\bforeach~ p\in \mathit{packetSeen}(m)$ do \\
\>\>\> $\bforeach~ q\in \mathit{reachableStates}(m)$ do \\
\>\>\>\> $\bforeach~ \gV{q'\,O'}\in \delta(q,p)$ do \\
\>\>\>\>\> $\mathit{reachableStates}(m)$ := $\mathit{reachableStates}(m)\cup \{q'\}$ \\
\>\>\>\>\> $\bforeach~ \gV{p'\,m'}\in O'$ do \\
\>\>\>\>\>\> $\mathit{packetSeen}(m')$ := $\mathit{packetSeen}(m')\cup \{p'\}$ \\
\>\>\>\>\> $\bif~ \babort(q')$ return failure \\
$\bif~ \babort(q')$ return success \\
\end{tabbing}
\caption{\label{fig:naive-alg}%
Fixed-point algorithm for computing the set of reachable states in a reverting network. \TODO{use the notation of the formal semantics of the execution of a single packet event instead of $\delta$}}
\end{figure}


\figref{naive-alg} presents a simple fixed-point algorithm for computing the set of reachable network configuration in the network. The algorithm uses the relation $\mathit{packetSeen}$ to store all the packets seen by each middlebox, and the relation $\mathit{reachableStates}$ to store all the state visited by each middlebox.

Upon reaching a fixed-point, $\mathit{packetSeen}$ stores exactly the set of packets that can be transmitted in the network, and $\mathit{reachableStates}$ stores exactly the set of reachable states of all middleboxes in the network.

Furthermore, since both $\mathit{packetSeen}$ and $\mathit{reachableStates}$ grow monotonically and their domains are finite the algorithm is guaranteed to terminate.
}

While the complexity of finding a least fixed point improves upon previous complexity results~\cite{velner2016some}, it is nonetheless exponential in the number of hosts in the network. In \secref{packet-effects} we present an abstract domain for which the least fixed point computation is polynomial in the number of hosts.


==> locality.tex <==
\subsection{Locality of Packet-Effect Middlebox Transitions}
\label{sec:local-sem}

An execution of an operation $\text{r}(\overline{a})~ \textbf{:=} \textit{cond}$,
in the context of processing an input packet $p$,
potentially updates the packet states of all packets.
However, for each packet $\tilde{p}$, the updated packet state $\tilde{s}'(\tilde{p})$
depends only on its pre-state $\tilde{s}(\tilde{p})$, the input channel $c$, the input packet $p$,
and $\tilde{s}(p)$, which determines the value of queries;
it is completely independent of the packet states of all other packets.
Since, in addition, the execution path of the middlebox when processing input packet $p$ depends only on the packet state of $p$, this form of \emph{locality}, which we formalize next, extends to entire middlebox programs as well.

Recall that each middlebox $m$ is associated with a program, $\prog(m)$,
given by an abstract syntax tree (AST). An evaluation of a program $\prog(m)$, for a given input packet,
is performed by a single recursive traversal of the AST (as there are no looping constructs) where some of the
branches non-deterministically choose a child node.
We can make the evaluation deterministic by adding a vector $\bar{n} \in {\N}^{*}$ as a parameter,
to indicate the child nodes to be taken at non-deterministic branches.
The vector is taken from the finite set $\paths(m)\eqdef\{n_1\ldots\ n_k \mid k=|\prog(m)| \land 1\leq n_i \leq k\}$.
%
We write %$\Meval[m](\tilde{s},p, c,\bar{n})=(\tilde{s}',(p_i, c_i)_{i=1..k})$,
$\tilde{s} \TrMPackM{(p, c)/(p_i, c_i)_{i=1..k},\bar{n}} \tilde{s}'$
if $\tilde{s} \TrMPackM{(p, c)/(p_i, c_i)_{i=1..k}} \tilde{s}'$ is a transition corresponding to the evaluation
of $\prog(m)$ with the deterministic choices given by the vector $\bar{n}$.
Note that in \AMDL, the path in the AST taken when evaluating $\prog(m)$ on input packet $p$ depends only on $p$, the packet-state of $p$, and $\bar{n}$.

\cbstart
\begin{example}
In the previous example, the transition from $\tilde{s}$ to $\tilde{s}'$ follows the path $\bar{n}=1, 2$.\qed
\end{example}

%A transition $\tilde{s} \TrMPack{(p, c)/(p_i, c_i)_{i=1..k}, \bar{n}} \tilde{s}'$ holds if
%$\tilde{s} \TrMPack{(p, c)/(p_i, c_i)_{i=1..k}} \tilde{s}'$ is a transition following the deterministic
%choices given by the vector $\bar{n}$.

\begin{definition}[Substate]
Let $\tilde{s} \in P\rightarrow Q(m)\rightarrow\{\True,\False\}$ be a packet effect state. We denote by $\tilde{s}|_{\{p,\tilde{p}\}} \in \{p,\tilde{p}\}\rightarrow Q(m)\rightarrow\{\True,\False\}$ the \emph{substate}
obtained from $\tilde{s}$ by dropping all packet states other than those of $p$ and $\tilde{p}$.
%
Let $\PState[m,p,\tilde{p}] \eqdef \{p,\tilde{p}\}\rightarrow Q(m)\rightarrow\{\True,\False\}$ denote the set of
substates for a pair of packets $p$ and $\tilde{p}$.
\end{definition}

\begin{example}
\label{examp:substate}
Consider the states $\tilde{s}$ and $\tilde{s}'$ used in \exref{packet-transition}
and the packets $p=(h_1,h_2,0)$ and $\tilde{p}=(h_2,h_1,0)$.
Then, using the shorthand notations of \tabref{PacketSpaceEnumeration}, we have the
following:
\[
\begin{array}{rcl}
\tilde{s}|_{\{p,\tilde{p}\}} &=& [p\mapsto(F,F,F), \tilde{p}\mapsto(F,F,F)]\\
\tilde{s}'|_{\{p,\tilde{p}\}} &=& [p\mapsto(F,F,F), \tilde{p}\mapsto(F,F,T)] \enspace.
\end{array}
\]
\qed
\end{example}

\begin{definition}[Substate transition relation]
We define the \emph{substate transition relation}\\
$\TrMPackSub{(p, c)/(p_i, c_i)_{i=1..k}, \bar{n}} : \PState[m,p,\tilde{p}] \times \PState[m,p,\tilde{p}]$ as follows.
%
A \emph{substate transition}\\
 $\tilde{s}[p,\tilde{p}] \TrMPackSub{(p, c)/(p_i, c_i)_{i=1..k}, \bar{n}} \tilde{s}[p,\tilde{p}]'$ holds if for every packet state $\tilde{s}$ such that
$\tilde{s}|_{\{p,\tilde{p}\}}=\tilde{s}[p,\tilde{p}]$,
we have that $\tilde{s} \TrMPack{(p, c)/(p_i, c_i)_{i=1..k}, \bar{n}} \tilde{s}'$ and $\tilde{s}'|_{\{p,\tilde{p}\}}=\tilde{s}[p,\tilde{p}]'$.
\end{definition}

\begin{example}
Continuing with the definitions in \exref{substate} and $\bar{n}=1,2$,
we have the following substate transition for $\fw_1$:
\[
\tilde{s}|_{\{p,\tilde{p}\}} \TrMPackSub{(p, \overset\rightarrow{e_2})/(p, \overset\rightarrow{e_3}), \bar{n}} \tilde{s}'|_{\{p,\tilde{p}\}} \enspace.
\]
Notice that in this case, since no query was made, the output substate is obtained by
propagating the packet state of $p$ and updating the packet state of $\tilde{p}$, independent of any other packet states.
\qed
\end{example}

\begin{definition}[2-Local Middlebox Semantics]
A middlebox semantics is \emph{2-local} if, for every packet $p$,
the following holds:
\[
\tilde{s} \TrMPack{(p, c)/(p_i, c_i)_{i=1..k}, \bar{n}} \tilde{s}' \;\;\Longleftrightarrow\;\;
\forall  \tilde{p}  \;.\; \tilde{s}|_{\{p,\tilde{p}\}} \TrMPackSub{(p, c)/(p_i, c_i)_{i=1..k}, \bar{n}} \tilde{s}'|_{\{p,\tilde{p}\}}
 \enspace.
\]
\end{definition}
\cbend

\begin{theorem}
The \AMDL\ packet effect semantics \iflong(\appref{amdl-semantics}) \fi is 2-local.
\end{theorem}

Furthermore, the substate transition relation, $\TrMPackSub{(p, c)/(p_i, c_i)_{i=1..k}, \bar{n}}$, can be computed directly from the code (without first computing the transition relation and then using projection)
in time linear in the size of the middlebox program. This is an even stronger notion of locality, which will be important later to efficiently compute a network-level abstract transformer (\secref{cartesian-packet}). 

==> lower.tex <==
\section{Complexity Lower Bounds} \label{sec:lower}

\TODO{wrote something. improve? The location doesn't seem good to me. It interrupts the flow.}
%\TODO{SH: move these two theorems to section on "lower bounds"}
The complexity of safety verification of stateful networks with respect to the unordered semantics has been investigated in~\cite{velner2016some}, where it is shown that:

\begin{theorem}~\cite{velner2016some}
\label{thm:unordered-tacas}
The safety verification problem for unordered (non-reverting) networks
is EXPSPACE-complete.
\end{theorem}
\TODO{need to explain what the parameters of the complexity are. Need to be careful since there we didn't have AMDL. }

In this work, we develop an abstract interpretation that is sound with respect to any semantics, but for unordered reverting networks it is also complete.
Completeness with respect to the ordered reverting semantics cannot be expected due to the following theorem:
\begin{theorem}
\label{thm:RevertingUndecidable}
The safety verification problem for ordered reverting networks
is undecidable.
\end{theorem}

In addition, the next theorem provides a lower bound on the complexity of any algorithm for safety verification, and in particular for our sound and complete abstract interpretation.
It shows that, under the assumption that P$\neq$NP, our algorithm is essentially optimal. \TODO{SH: rephrase?}
\begin{theorem}
\label{thm:reverting-unordered-conphard}
The safety problem for  unordered reverting networks is coNP-hard.
\end{theorem}
\TODO{SH: not sure what the parameters of the complexity are. The proof mentions the number of queries. This was not yet mentioned.
Perhaps this is an argument against first defining the network semantics and only then AMDL and middlebox semantics.
An alternative is to move this theorem to the section on abstract interpretation after analyzing the complexity to show the result is tight.}



==> overview.tex <==
\section{Overview}
\label{sec:overview}
This section provides an informal overview of our approach.

\newcommand{\fw}{\textit{fw}}
\newcommand{\type}{\texttt{type}}
\newcommand{\is}{\textit{is}}
\newcommand{\requested}{\texttt{requested}}
\newcommand{\trusted}{\texttt{trusted}}

%\para{A Running Example}
\subsection{A Running Example}
%\subsection{Stateful Networks \texorpdfstring{$\approx$} ~ Message Passing Programs}
%
%The theme of this paper is developing a scalable algorithm for verifying the safety of a network
%which contains not only normal switches but also stateful middleboxes.
%Middleboxes contain mutable states which record the history of forwarded packets.
%The state of a middlebox affects its forwarding behavior which ultimately affects the states of
%other middleboxes when the forwarded packet (message) is received.
%
%Technically, a network with stateful middleboxes can be viewed as a special kind of a message passing program
%where processes simulate the behavior of nodes in the network and packets (messages) are sent via asynchronous channels
%which emulate ports.
%The process at each node describes the behavior of a middlebox.
%%Processes describing hosts merely generate packets.
%%\TODO{need to say that they also describe hosts. Problem is that the rest of the description only refers to middlebox processes}
%Processes describing middleboxes can have local mutable states implemented using relations which record the ``local'' state of the network based on
%the packets seen so far.
%The code at each middlebox process reacts to packets in the incoming channels by
%(i)~forwarding potentially modified packets to other channels
%(ii)~changing its internal state,
%and optionally (iii)~reporting a violation of a safety property (using an ``abort'' command).
%
%In this setting, we can view switches as a degenerate case of middleboxes with immutable states.
%
% \begin{figure}
%   \centering
%   \includegraphics[width=0.45\textwidth]{img/running-ex}
%   \caption{Network topology for the running example.}
%   % The network contains two hosts, $h_1$ and $h_2$, two session firewalls $fw_1$ and $fw_2$, and a property middlebox $is$ that monitors isolation
%   % between the hosts.}
%   \label{fig:running-ex-topo}
% \end{figure}
%
%\lstset{numbers=left,numbersep=-7pt}
%
%\begin{figure}
%    \begin{subfigure}[b]{0.48\textwidth}
%        \centering
%        \begin{footnotesize}
%        \begin{lstlisting}[mathescape=true]
\begin{figure}
\centering
\begin{subfigure}[b]{0.4\textwidth}
% \begin{center}
\begin{footnotesize}
\begin{alltt}
\begin{tabbing}
sf\=irewall = do \+ \\
in\=ternal_port ? p => \+ \\
if\= \+\\
p.dst in trusted => external_port ! p\\
\(\Box\) \\
p.\=type = 0 => // request packet \+ \\
external_port ! p; \\
requested(p.dst) := true \-\-\\
fi \-\\
\(\Box\)\\
ex\=ternal_port ? p => \+ \\
if\= \+ \\
p.src in trusted => internal_port ! p\\
 \(\Box\)\\
p.\=type = 1 and p.src in requested => \+\\
// response packet with a request\\
trusted(p.src) := true \- \- \\
fi \-\- \\
od
 \end{tabbing}
 \end{alltt}
 \end{footnotesize}
  % \end{center}
  \caption{\label{fig:session-fw-code}%
  \AMDL\ code for $\fw_1$ and $\fw_2$.}
\end{subfigure}
\qquad
\begin{subfigure}[b]{0.4\textwidth}

 \begin{subfigure}[b]{\textwidth}
  % \centering
  \includegraphics[width=\textwidth]{img/running-ex}
  \caption{A network topology.}
  % The network contains two hosts, $h_1$ and $h_2$, two session firewalls $fw_1$ and $fw_2$, and a property middlebox $is$ that monitors isolation
  % between the hosts.}
  \label{fig:running-ex-topo}
 \end{subfigure}
\par\bigskip
\par\bigskip
\par\bigskip
\par\bigskip
% \begin{center}
\begin{subfigure}[b]{\textwidth}
\begin{footnotesize}
\begin{alltt}
\begin{tabbing}
is\= = do \+ \\
ex\=ternal_port ? p =>\+\\
if\= \+ \\
p.src = forbidden => abort\\
\(\Box\)\\
true => internal_port ! p \-\\
fi \- \\
\(\Box\)\\
in\=ternal_port ? p => \+ \\
true => external_port ! p \-\- \\
od
\end{tabbing}
\end{alltt}
\end{footnotesize}
% \end{center}
\caption{ \label{fig:safety-code}%
\AMDL\ code for $\is$.}
% The code forwards all packets in one direction and drops packets from
% forbidden hosts and aborts.}
 \end{subfigure}
 \end{subfigure}
\caption{Network topology and \AMDL\ code for the running example.}
 \end{figure}
%
%\begin{example} \Cref{fig:running-ex-topo} depicts the topology of
\figref{running-ex-topo} shows a simple network where two stateful
firewalls are connected in a row to prevent traffic \cbstart between nodes $h_2$
to $h_1$.
This is an artificial example meant to illustrate the verification process. \cbend
More realistic examples are
presented in \secref{empirical}. It is assumed that hosts $h_1$
and $h_2$ can send and receive arbitrary packets on channels $e_1$
and $e_4$, respectively. The example is implemented using three
middleboxes: two middleboxes, $\fw_1$ and $\fw_2$, running firewalls
that restrict traffic from left to right and from right to left,
respectively, and one middlebox, $\is$, checking whether isolation
between $h_2$ and $h_1$ is preserved. In $\fw_1$, $e_2$ is connected
to the ``internal'' port and $e_3$ is connected to the ``external''
port, thus limiting traffic from right to left. In \cbstart $\fw_2$, $e_4$ is
connected to the ``internal'' port and $e_3$ \cbend is connected to the
``external'' port, thus limiting traffic from left to right. In $\is$,
$e_1$ is connected to the ``internal'' port and $e_2$ is connected
to the ``external'' port.

\figref{session-fw-code} describes the code running in either of
the session firewalls, $\fw_1$ and $\fw_2$. We use CSP/OCCAM-like syntax
where (messages) packets are sent/received asynchronously. The
middlebox non-deterministically operates on a packet from the
``internal'' port  or the ``external'' port. When reading a packet
from the ``internal'' port, the program distinguishes between two
cases. In the first case, a session had been previously established, and
the packet is simply forwarded to the ``external'' port.
%
In the second case the type of the packet is a ``request'' packet (\type=0), and the program adds the destination host to the set of
\verb|requested| hosts and forwards the ``request''. The
\verb|requested| set is used to store the hosts to which the
middlebox sent a ``request'' packet, to avoid the case where a
session is established with a host that the middlebox did not send a
``request'' to. Packets that do not fall into any of these two cases
are discarded with no further processing.

When the middlebox reads a packet from the ``external'' port again
it distinguishes between two cases --- in one case a session had
previously been established, and is similar to its ``internal''
counterpart.
In the second case, the processed packet is a ``response'' packet (\type=1) from a host that is in the \verb|requested| set, and the program marks the source of the packet as \verb|trusted|, thus establishing a session.
Other packets are discarded.

\cbstart
A ``data'' packet (\type=2) is implicitly handled by checking whether the source/destination of the packet is in the \texttt{trusted} set,
and if so, allowing the packet to propagate on.
\cbend

\figref{safety-code} describes the code running in a special middlebox, $\is$, which
intercepts packets before they arrive to host $h_1$ ---
the middlebox non-deterministically reads a packet from the ``external'' port and aborts
if the source of the packet is the host $\texttt{forbidden} = h_2$, and otherwise forwards to $h_1$ on the ``internal'' port.
On the other direction, it simply forwards packets from the ``internal'' port to the ``external'' port.
%
\cbstart In this example, $\is$ models the safety property. \cbend
%\end{example}

%
%\subsection{Order of Packet Abstraction}
%In \cite{velner2016some},
%it is shown that the problem of proving safety for stateful
%middleboxes is undecidable even for finite state middleboxes and
%even when the topology is fixed. The reason is that sequences of
%packets can simulate the tape of a Turing machine. Therefore, we
%apply abstract interpretation in order to obtain a sound and
%potentially incomplete verification. We define an approximate
%semantics for messages passing programs which overapproximates
%network behavior by assuming that the order of packet processing by
%a process is independent of the order in which packets arrived.
%Technically, this means that channels contain multisets of packets
%and the middlebox reacts to one of the packets in the incoming
%channel by removing it from the multiset and taking its action. In
%our preliminary experience this abstraction does not lose precision
%in many cases. Moreover, since packets are processed atomically,
%order of processing can be enforced via handshaking between
%processes.


\subsection{Modular Network Verification}
%\para{Modular Network Verification}
Unfortunately, as shown by ~\cite{velner2016some}, the complexity of
checking safety is hard even when the order of packets on channels is ignored.
The complexity stems from the potential interactions between states
of middleboxes and received packets.

In this paper, we suggest the first fully automatic modular method for verifying safety
of stateful networks.
%The safety of each middlebox is proven in a circular way assuming something about the other middleboxes.
Technically, it is a Cartesian abstract interpretation~\cite{cousot1979systematic,DBLP:journals/tcs/FlanaganFQS05,POPL:JMP17}
that combines network-level abstractions and middlebox-level abstractions.

We first explain our network-level abstractions.
Our method abstracts away correlations between the local states of
individual middleboxes and the contents of the individual channels. In
addition, the contents of channels are abstractly represented
as \emph{sets} of packets (rather than sequences). %multisets).


\begin{table*}
\begin{footnotesize}
\[\arraycolsep=2pt
\begin{array}{|c | c | c | c |  c | c | c | c| c | c | l|}
\hline \mathbf{\overset\rightarrow{e_1}} & \mathbf{\overset\leftarrow{e_1}}
& \mathbf{\overset\rightarrow{e_2}} & \mathbf{\overset\leftarrow{e_2}} &
\mathbf{\fw_1} &  \mathbf{\overset\rightarrow{e_3}} &
\mathbf{\overset\leftarrow{e_3}} & \mathbf{\fw_2}  &
\mathbf{\overset\rightarrow{e_4}} & \mathbf{\overset\leftarrow{e_4}} & \textbf{action} \\
\hline \hline
\begin{array}{l}
p_{(1,2,0)}\\
p_{(1,2,1)}\\
p_{(1,2,2)}\end{array} & \emptyset & \emptyset & \emptyset &
 (\emptyset, \emptyset) &
\emptyset & \emptyset & (\emptyset, \emptyset) & \emptyset
&
\begin{array}{l}
p_{(2,1,0)}\\
p_{(2,1,1)}\\
p_{(2,1,2)}\end{array}
 & \text{initial state} \\
\hline
& & p_{(1,2,0)} & & & & & & & & \textit{is} ~\text{reads}~ p_{(1,2,0)}\\
\hline
& &
\begin{array}{l}
p_{(1,2,0)}\\
p_{(1,2,1)}\end{array}
& & & & & & & & \textit{is} ~\text{reads}~ p_{(1,2,1)}\\
\hline
& &
\begin{array}{l}
p_{(1,2,0)}\\
p_{(1,2,1)}\\
p_{(1,2,2)}\end{array}
& & & & & & & & \textit{is} ~\text{reads}~ p_{(1,2,2)}\\
\hline
&  &  &  & \begin{array}{l}
(\emptyset, \emptyset)\\
(\{h_2\}, \emptyset)
\end{array}
& p_{(1,2,0)} & & & & & \textit{fw}_1~ \text{reads}~ p_{(1,2,0)}\\

\hline

& & & & & & & & & & \textit{fw}_1~ \text{reads}~ p_{(1,2,1)}\\

\hline

& & & & & & & & & & \textit{fw}_1~ \text{reads}~ p_{(1,2,2)}\\

\hline

& & & & & & p_{(2,1,0)} &
\begin{array}{l}
(\emptyset, \emptyset)\\
(\{h_1\}, \emptyset)
\end{array}
& & & \textit{fw}_2~ \text{reads}~ p_{(2,1,0)}\\

\hline

& & & & & & & & & & \textit{fw}_2~ \text{reads}~ p_{(2,1,1)}\\

\hline

& & & & & & & & & & \textit{fw}_2~ \text{reads}~ p_{(2,1,2)}\\

\hline

& & & & & & & & & & \textit{fw}_1~ \text{reads}~ p_{(2,1,0)}\\

\hline

& & & & & & & & & & \textit{fw}_2~ \text{reads}~ p_{(1,2,0)}\\

\hline
\hline
\end{array}
\]
\end{footnotesize}
\caption{\label{tab:CartesianExplicit}%
Modular analysis of the running example with explicit state
representation. Only changed values are shown.
The abstract states of channels are sets.
The abstract states of firewalls are sets of pairs for the values of
the \texttt{requested} and \texttt{trusted} sets. Each cell in the table represent a set of the elements described within, except for empty sets in the initial state.
The notation $p_{(i,j,k)}$ stands for the packet from $h_i$ to $h_j$ with type $k$.
}
\end{table*}

\begin{example}
\label{examp:cartesian-explicit}
\tabref{CartesianExplicit} shows the
run of our analysis, when restricted to the network-level abstractions, on the running example.
Each row corresponds to a step in the least fixpoint computation of the (abstract) reachable network states.
Each column at the table represents the abstract content of a channel
(as a set of packets)
or the abstract state of an individual middlebox (as the contents of its set-valued variables).
For each channel $e$, $\overset\rightarrow{e}$ denotes channels connecting traffic from left to the right, while
%For each channel $c$,
$\overset\leftarrow{e}$ denotes channels connecting traffic from right to the left.
For example, $\overset\rightarrow{e_1}$ contains packets sent from $h_1$ to $\is$.

\cbstart
Channel abstract states are sets of packets. %\TODO{not clear. Last time they were mentioned they were multisets.}

For the firewall middleboxes, a (concrete) state is a pair of values for the \verb|requested| and \verb|trusted| sets.
An abstract state is a set of such (concrete) states.
%
The isolation middlebox is stateless.

At the initial configuration, the states of $\fw_1$ and $\fw_2$ are pairs of empty sets;
the states of channels $\overset\rightarrow{e_1}$ and $\overset\leftarrow{e_4}$ are all the packets that hosts $h_1$ and $h_2$
can send, respectively.

The analysis ignores the correlations between different columns.
At each step, the analysis chooses an input channel and a middlebox state and computes the next state.
The analysis stops when no more new middlebox states or channel states are discovered and reports potential violation of the safety
property if the \texttt{abort} command is executed.
\cbend
\qed
\end{example}

%\para{Reasoning about Cartesian Abstractions}
\subsection{Reasoning about Cartesian Abstractions}

The abstract transformer~\cite{cousot1979systematic} obtained by the network-level abstraction discussed so far can be computed on the fly by: (1) computing the sets of configurations represented by a given input channel and
current set of states, (2) applying middlebox code to each potential
packet in the set and each state, and then (3) projecting
the relevant new column(s). %\TODO{should we emphasize that we just need to concretize two columns: middlebox state and channel and not all? Something like: }
%\TODO{The use of `column' here is not clear. The table hasn't been discussed yet.}
%%% ADDED
Since middlebox behavior only depends on its own state, the computation can be performed locally by concretizing its own state and its adjacent channel states,
without considering a concretization of the entire network state.
%This abstraction is called Cartesian since it computes the cartesian products of the accumulated behaviors of each process.
%This is similar to thread-modular analysis, e.g., \cite{POPL:JMP17}.
%Notice that modularity does not imply that each middlebox assumes arbitrary behavior from the environment.

%\TODO{need to somehow explain why this also makes the state of channels a set and not a multiset. -- this is actually an additional abstraction that is missing here.}


\begin{example}
Consider \tabref{CartesianExplicit} again.
In the first action, the code of $\is$ executes and reads
$(h_1, h_2, 0)$ from $\overset\rightarrow{e_1}$. Notice that this does not
change the (abstract) content of this channel. The packet is
forwarded to $\overset\rightarrow{e_2}$. Thus, our analysis only accumulates
packets, ignoring their order. The reachable states of the
middleboxes are explicitly maintained. For example, when $\fw_1$
reads $(h_1, h_2, 0)$ from $\overset\rightarrow{e_2}$, it forwards it to
$\overset\rightarrow{e_3}$ and reaches a new state with
$\texttt{requested}=\{h_2\}$ and $\texttt{trusted}=\emptyset$.

Notice that in this example, the analysis proved that the \texttt{abort}
command can ever be executed on arbitrary packet propagation scenarios.
Specifically, no packets ever reaches channel
$\overset\leftarrow{e_2}$, so the safety middlebox $\is$ never
reads a packet that will result in the execution of an \texttt{abort}
command. Thus, the analysis succeeded in proving isolation.

\cbstart
This example illustrates that, although our analysis employs Cartesian abstraction,
it is able to prove a network-wide property. Specifically, proving isolation requires
reasoning about the states of both firewalls.
%
We note that removing either of the firewalls violates the safety property. \cbend
\qed
% \TODO{Explain more clearly.}
%In the example presented in \Cref{fig:running-ex-topo} our abstraction ignores the correlations between the contents of the \verb|trusted| and \verb|requested| relation in the middleboxes $fw_1$ and $fw_2$, as well as the correlations between the state of individual processes and the state of the communication channels.

%The analysis computes the set of packets that can be sent by the hosts to the firewalls. The contents of the incoming channels of the firewalls will then provide the `environment' assumptions for the analysis of the firewall. The analysis of each firewall will compute the request packet sent from either firewall to the other, and add firewall states with relevant hosts to the set of reachable states.
%The addition of request packet to each firewall's incoming channel changes the environment assumptions for the analysis of the firewalls, but the additional assumptions do not lead to new packets or new states.
%The analysis does not find any packets from $h_1$ leading to $h_2$, and successfully proves that the network is safe.
\end{example}

%\para{Reverting Systems}
\subsection{Reverting Systems}

Our network-wide modular verification may fail to prove safety for systems in which the safety depends on correlated states.
Therefore, we tried to characterize the systems in which Cartesian
abstraction does not lose information.
One class of systems for which this Cartesian abstraction does not lose precision is the class of
\emph{Reverting Systems}, which bares some similarity with the notion of soft states in networks~\cite{raman1999model}.
A \emph{reverting system} is a system in which every middlebox may non-deterministically revert to its initial
state at any point in time.

We show that in reverting systems where, in addition, packets are processed in an arbitrary order, if a packet is received at some middlebox state, it can be received when that middlebox is at any
reachable state. This allows us to prove that the Cartesian abstraction is precise for reverting systems with unordered channels.

\ignore{
Moreover, a reachable middlebox state can be reached when the other middleboxes are in any other reachable state.
Therefore, in reverting systems any combination of reachable states for the different middleboxes and channels is itself
reachable, which means that the Cartesian abstraction is precise for reverting systems.\footnote{In fact, not every combination of reachable channel states is indeed reachable, but
every packet can be received with any combination of middlebox states, which suffices to ensure precision of the abstraction for safety.}
%\TODO{imprecise, but I can live with that. For the channels, it's not every combination. If we had it, then we would have $\gamma$-completeness. Added footnote to overcome this}
\TODO{we don't actually show that. need to rephrase our completeness}
}

%\begin{example}
In the example presented in \figref{running-ex-topo} the Cartesian abstraction is precise w.r.t. to the safety property.
The network in the example is safe, and indeed, even if we add revert transitions to the network, there is no history in the network that leads to executing an \verb|abort| command.
Intuitively, this is because after one of the firewalls in our example reverts to its initial state, its forwarding behavior can only ``shrink'',
so after the revert it will return to a state in which it can only send ``request'' packets to the ``external'' port and no packets to the
``internal'' port.
In our example, the only way a firewall would permit a packet from $h_2$ to reach $h_1$ is if a ``response'' packet had
been sent beforehand, which cannot happen in the network, regardless of whether the firewalls revert to their initial state or not.
%\end{example}

\para{Packet State for Polynomial Safety Checking}
The complexity of checking safety with the network-level Cartesian  abstraction is polynomial in the number of middlebox states.
However, the number of middlebox states is exponential in the number of hosts in the system, which means that it will be hard
to scale this approach to realistic systems with a large number of hosts.
For example, in the case of firewalls with potentially $k$ trusted hosts, the number of states is $2^k$.

To deal with the explosion that arises from the  state-space of the middleboxes, we employ a middlebox-level abstraction.
%Fortunately,
We observe that the middlebox behavior for many real middleboxes can be expressed in a way that makes verification tractable.
The idea is that middlebox behavior is local in the following way: we can view a single middlebox state as a mapping from packets to their \emph{packet states}, where the packet state of $p$ suffices to determine both the sequence of packets that the middlebox outputs when it receives $p$ as an input packet, and the way the state changes in response to $p$.
Formally, this defines a bisimilar representation of the middlebox states, which is facilitated by our language for describing middleboxes.
%%The idea is that we do not need to explore \emph{all} middlebox states to prove safety.
%%Instead, we observe that two states which `affect' packets in the same way are bi-similar.
%and leads to (effectively) polynomial-time modular verification which performs Cartesian abstraction using the packet state representation for
%middlebox states. The latter is facilitated by our language for describing middleboxes.

In \secref{amdl}, we define a simple programming language --- \textbf{A}bstract \textbf{M}iddlebox \textbf{D}efinition
\textbf{L}anguge (\AMDL) --- for defining the effect of middleboxes.
Intuitively, we restrict the ability of the middlebox to generate new packets.
The code can only rewrite packets using values of the current processed packet or configuration constants.
For example, swapping source and destination is allowed but adding one to destination is forbidden.
The effect of a packet on the state is restricted in a similar way. %, by only allowing to add or remove packet fields and constant from relations.
We show that the effect of many interesting middleboxes can be defined in this language.

In \secref{abs-int} we utilize \AMDL\ for defining a novel (effectively) polynomial-time modular verification, which performs Cartesian abstraction using the packet state representation for
middlebox states.
%polynomial-time verification algorithm for checking safety.
%The algorithm does not lose precision with respect to the explicit state enumeration. Hence it is also  precise for reverting unordered networks.
Instead of tracking middlebox states as valuations of relations, the algorithm tracks, for each packet header,
the potential packet states. Technically, packet states are the valuations of the Boolean conditions in the code (also code state queries) that match the packet.
Each of these valuations uniquely determines the potential forwarded packets and new state.
\input{packet-space-table}

\begin{example}
\tabref{PacketSpaceEnumeration} shows the verification process with packet states in the running example.
Instead of storing the contents of relations \verb|trusted| and \verb|requested| in each middlebox state,
\cbstart we store, for each packet, whether each of the expressions
``\verb|p.dst in trusted|'', ``\verb|p.src in trusted|'', and ``\verb|p.src in requested|'',
evaluates to \True\ ($T$) or \False\ ($F$), respectively.

Since both relations are empty in the initial state, the packet states for both firewalls map each packet
to $(F,F,F)$.

Recall that when $\fw_1$ reads $(h_1, h_2, 0)$ from $\overset\rightarrow{e_2}$, it forwards it to
$\overset\rightarrow{e_3}$ and reaches a new state with $\requested=\{h_2\}$ and $\trusted=\emptyset$.
%
Therefore, any future evaluation of the expression ``\verb|p.src in requested|'' (for any value of \type)
should result in \True.
%
Under the packet state representation, this would result in adding to the abstract state of $\fw_1$ a packet state
similar to that of the initial state where each of the packets
$p_{(2,1,0)}$, $p_{(2,1,1)}$, and $p_{(2,1,2)}$ is re-mapped from $(F,F,F)$ to $(F,F,T)$.
%
Our middlebox-level Cartesian abstraction allows us to instead accumulate these mappings (separated by a horizontal line
from the initial mappings) in a single abstract state, \emph{without affecting the overall precision of
the abstract interpretation}.

A similar change to the packet state of $\fw_2$ occurs upon reading the packet $(h_2, h_1, 0)$ from $\overset\leftarrow{e_4}$.
\qed
\cbend
\end{example}

%Technically, we define a set of packet states and show that it is bisimilar to the concrete states w.r.t.
%the safety property.
%Also, the
The size of the packet state space is quadratic in the number of hosts, and exponential in the number of Boolean conditions that examine relations in the code. The latter is typically a constant \cbstart(three, in our example)\cbend, which  gives us a polynomial time algorithm for safety checking.
%This algorithm is precise for reverting networks under the order abstraction.
%
Also, for reverting unordered networks, the algorithm does not lose precision with respect to the middlebox state enumeration. Hence it is also precise for such networks.

%We implemented our approach on top of LogicBlox~\cite{aref2015design} and report on preliminary results.
%Therefore, we propose an alternative approach to representing the state of individual processes.
%Instead of explicitly representing the state of a process we map each potential packet in the system to the potential
%boolean exresults we would get if
%we evaluated each one of the various boolean expressions in the process for that packet.
%We show that this state representation is bisimilar to the explicit state representation, and
%consequently safety checking in the message space is sound and precise.

%\subsection{False Alarms}
%The cartesian abstraction may be imprecise for not reverting networks.
%In this case a more refined algorithm which tracks correlations between middlebox states.
%\TODO{Give an example}

\figref{CombinedAbstractions} provides a high-level view of the different (abstract) semantics introduced in the sequel.

\begin{figure}
  \centering
  \begin{tabular}{|c|}
  \hline
  Cartesian network domain over Cartesian packet space domain:\\
  $M\rightarrow (P\rightarrow \pow{Q\rightarrow \{\True,\False\}}) \times (E\rightarrow \pow{\Pi})$\\
  \hline\\
  \includegraphics[width=0.99\textwidth]{img/CombinedAbstractions}\\
  \hline
  \end{tabular}
  \caption{Hierarchy of abstractions.
  Solid edges stand for abstraction (either by relaxing the
  transition relation or by abstracting the configurations).
  Dashed edges stand for instantiation of the middlebox
  (local) semantics.}
  \label{fig:CombinedAbstractions}
\end{figure} 

==> reverting.tex <==
\subsection{Unordered Network Semantics}
\label{sec:unordered-semantics}

The first relaxed semantics that we define allows channels not to preserve the packet transmission order. Namely, packets in the same channel may be processed in a different order than the order in which they were received.

\ignore{
\para{Unordered Network Configurations}
\TODO{keep configurations the same. Move this to abstraction section}
An \emph{unordered network configuration} $\Sigma^u = (M\to \Sigma[M])\times(E \to \mset{P})$
assigns communication channels to multisets of packets, thus abstracting away the order
between packets.
%
The set of \emph{Unordered configurations} is defined as $\Sigma^u = $. \TODO{complete}

We denote the unordered initial state by $(\sigma_I,\lambda\,e\in E\,.\, \lambda\,p\in P\,.\, 0)$,
where $\sigma_I$ denotes the initial state of all middleboxes.
}

\para{Unordered Network Transitions}
%\TODO{say that this is the best transformer}
The unordered network  semantics is given by the transitions
$(\sigma,\pi) \TrN{p,e,m}{u} (\sigma',\pi')$, where all conditions are as in the case of ordered transitions, with the exception of condition (i) that changes as follows:
%We define the unordered semantics of a transition in the network as $(\sigma,C) \xrightarrow{p,e,m}_u (\sigma',C')$ similarly to the definition of ordered transitions, except that condition (i) changes to:
(i) $p$ is \emph{some} packet on the channel $e \in E$. Namely, a transition can be triggered by \emph{any} packet on the ingress channel of a middlebox.
%Error transitions are also adapted similarly.
Host transitions remain unchanged.

\ignore{
We define the unordered semantics of a transition in the network as $(\sigma,C) \TrN{p,e,m}{u} (\sigma',C')$ where
the following hold:
(i) $p$ is \emph{some} packet on the channel $e \in E$,
(ii) the channel $e$ is an ingress channel of middlebox $m$,
(iii) there exists a command $c$ in middlebox $m$ s.t. $\sembr{c}_{pre}$ holds in state $\sigma(m)$ for packet $p$,
(iv) the safety condition $\msafe{m}$ of the middlebox $m$ holds for the middlebox state $\sigma(m)$ for packet $p$,
(v) $C'$ is the result of removing packet $p$ from the multiset assigned to channel $e$ and adding the result of $\sembr{c}_{out}$ to the the appropriate channels via multiset sum, and
(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.
}

The transformer, the collecting semantics, denoted $\BB{\Net}^u$, as well as
the safety verification problem for unordered networks are defined %in the same way as in the ordered case.
similarly to the ordered case.

\begin{theorem}~\cite{velner2016some}
\label{thm:UnorderedEXSPACE}
The safety verification problem for unordered networks
is EXPSACE-complete.
\end{theorem}

\subsection{Reverting Network Semantics}

The next relaxed semantics that we consider allows middleboxes to revert to their initial state after every transition.
%This semantics does not change the set of configurations, but increases the set of transitions to include reverting transitions.

\para{Reverting Network Transitions}
The ordered reverting network semantics is given by the transitions
$(\sigma,\pi) \TrN{p,e,m}{or} (\sigma',\pi')$, where all conditions are as in the case of ordered transitions, with the exception of condition (iii) that changes as follows:
(iii) $\sigma(m) \TrM{(p, e)/(p_i, e_i)_{i=1..k}} \sigma'(m)$ or $\sigma'(m) = \sigma_I(m)$, meaning that the middlebox $m$ may revert to its initial state.
%We define the ordered reverting semantics of a transition in the network as $(\sigma,C) \xrightarrow{p,e,m}_{or} (\sigma',C')$, where conditions (i)-(v) are as in the case of ordered transitions and condition (vi) changes as follows:
%(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
%$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.
The unordered reverting network semantics is defined similarly; the corresponding transitions are denoted $(\sigma,\pi) \TrN{p,e,m}{ur} (\sigma',\pi')$. %, is defined similarly.
%In both cases, error transitions remain unchanged.
In both cases, host transitions remain unchanged.


%We denote the transformers of ordered reverting networks and unordered reverting networks by $\Tr^{or}$ and $\Tr^{ur}$, respectively,
The transformers and the collecting semantics are defined as before. We denote by $\BB{\Net}^{or}$ the collecting ordered reverting semantics and by $\BB{\Net}^{ur}$ the collecting unordered reverting semantics.
The safety verification problem for these cases is adapted accordingly.

%\TODO{SH: move these two theorems to section on "lower bounds"}
\begin{theorem}
\label{thm:RevertingUndecidable}
The safety verification problem for ordered reverting networks
is undecidable.
\end{theorem}
%This theorem shows that the reverting semantics alone does not suffice to make safety verification tractable.

\begin{theorem}
\label{thm:reverting-unordered-conphard}
The safety problem for  unordered reverting networks is coNP-hard.
\end{theorem}

In \secref{abs-int}, we present an abstract interpretation algorithm that is both sound and complete for the unordered reverting semantics, and essentially meets the lower bound stated in  \Cref{thm:reverting-unordered-conphard}, as it is exponential in the number of state queries of any middlebox and polynomial in the number of middleboxes, hosts and packets.
%the combination of the unordered and the reverting semantics allows for an efficient abstract interpretation algorithm that is both sound and complete for the unordered reverting semantics.

%\TODO{RM: Why can't we be more specific? ...as it is exponential in the maximal number of queries of any
%middlebox and polynomial in the number of middleboxes, hosts, and tags.}


%However, as we show in the remainder of the paper, the combination of the unordered and the reverting semantics allows for an efficient abstract interpretation algorithm that is both sound and complete for the unordered reverting semantics.
%\TODO{SH: added this explanation. Is it ok?}

%
%\begin{theorem}
%\label{thm:reverting-unordered-conphard}
%The safety problem for  unordered reverting networks is coNP-hard.
%\end{theorem}
%\TODO{SH: not sure what the parameters of the complexity are. The proof mentions the number of queries. This was not yet mentioned.
%Perhaps this is an argument against first defining the network semantics and only then AMDL and middlebox semantics.
%An alternative is to move this theorem to the section on abstract interpretation after analyzing the complexity to show the result is tight.}

\ignore{
The reverting unordered semantics is
not directly implementable (the set of packet multisets is infinite).
We continue by proving and utilizing properties of the semantics,
which in later sections allow us to apply sound abstractions, while still maintaining
fixpoint-completeness, leading us to the
\emph{Cartesian network abstraction}.
}

%\TODO{add transitions such that: $\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.}

\para{Sticky Properties}
%\TODO{this is never used. Not sure why we include it. Maybe it gives intuition for the "first" Cartesian abstraction but in any case we don't stop there and don't claim anything about it.}
%\TODO{SH: remove this paragraph and move the intuition to the sticky property in the packet effect section}
\cbstart
Unordered reverting networks have two useful properties, which we define next --- the \emph{sticky states} property and the \emph{sticky packets} property --- that make the abstract interpretation described in \secref{abs-int} complete. \cbend
\ignore{
Intuitively, the sticky packets property states that if a packet is pending for a middlebox in some run of the network then any run has an extension in which the packet is pending again.
%n event occurs in some run of the network, then any run has an extension in which that event occurs.
%Consequently, disregarding the multiplicity of packets on the channels does not incur precision loss w.r.t. safety.
Consequently, it is not necessary to maintain the cardinality of every packet on every channel and
it is not necessary to maintain the correlation between a channel and the set of packets
that can simultaneously appear there.
Instead, it is sufficient to record, for each individual channel $e$ and individual packet $p$,
whether $p$ has arrived on $e$ at some point.
The sticky states property ensures that ignoring the correlation between the state of a middlebox $m$ and the channels connected to it does not lose precision (for safety).
This implies that one can also ignore correlations between the states of different middleboxes, making a Cartesian abstraction precise.
%and the states of other middleboxes as well as the states of the channels that are not connected to the middlebox $m$.
}


%The following lemma shows that the reverting unordered semantics
%maintains the sticky packet property.

\begin{lemma}[Sticky Packets Property]
\label{lem:sticky-packets}
For every channel $e$ and packet $p$:
If in some reachable configuration $e$ contains $p$, then every run can be extended such that $e$ will eventually contain $p$.
%
Moreover, every run can be extended such that $e$ will eventually contain $n$ copies of $p$ (for every $n>0$).
\end{lemma}
%\begin{proof}
%The proof relies on the reverting property and on the fact that the channels are unordered.
%
%Let $\sigma_0$ be a reachable configuration in which $p$ occurs in $e$, and let $s_0$ be the scenario that led to it, i.e., the sequence of events that took place.
%Consider an arbitrary run (scenario) $\pi$. One can extend $\pi$ with the following scenario:
%First all the middleboxes return to their initial state.
%Second, scenario $s_0$ occur, i.e., only packets from scenario $s_0$ are processed, and the other packets are ignored.
%This extension is possible because the channels are unordered.
%
%To construct a scenario in which $e$ contains $n$ copies of $p$, we just concatenate the above mentioned extension $n$ time.
%\end{proof}

The sticky packets property implies that, in verifying such networks, it is not necessary to maintain the cardinality of every packet on every channel and
it is not necessary to maintain the correlation between a channel and the set of packets
that can simultaneously appear there.
Instead, it is sufficient to record, for each individual channel $e$ and individual packet $p$,
whether $p$ has arrived on $p$ at some point, without losing precision w.r.t. safety.

%We now show that unordered reverting networks have the sticky states property.

\begin{lemma}[Sticky States Property]
\label{lem:sticky-states}
For every channel $e$, packet $p$, middlebox $m$ and state %$\sigma_m$
$s$ of $m$:
If, in some reachable configuration, channel $e$ contains $p$ and in some (possibly other) reachable configuration $m$ is in state %$\sigma_m$,
$s$, then %every run can be extended such that eventually we get to
there exists a reachable configuration where simultaneously $e$ contains $p$ and $m$ is in state $s$. % $\sigma_m$.
%If in some scenario channel $c$ contains $p$ and $m$ is in state $q_m$, then every scenario can be extended such that eventually we get to a configuration where simultaneously $c$ contains $p$ and $m$ is in state $q_m$.
\end{lemma}

%\begin{lemma}
%\label{lem:sticky}
%For every channel $e$, packet $p$, middlebox $m$ and state $\sigma_m$ of $m$:
%If in some reachable configuration channel $e$ contains $p$ and in some (possibly other) reachable configuration $m$ is in state $\sigma_m$, then every run can be extended such that eventually we get to a configuration where simultaneously $e$ contains $p$ and $m$ is in state $\sigma_m$.
%%If in some scenario channel $c$ contains $p$ and $m$ is in state $q_m$, then every scenario can be extended such that eventually we get to a configuration where simultaneously $c$ contains $p$ and $m$ is in state $q_m$.
%\end{lemma}
%\begin{proof}
%Let $(p_1,\dots,p_\ell)$ be the sequence of packets that $m$ processed from the latest reset until it arrives to state $\sigma_m$ in the given witness scenario.
%
%Consider an arbitrary run.
%By Lemma~\ref{lem:sticky_packets} we can extend this run such that $p_1,\dots,p_\ell$ are pending packets in the ingress channel of middlebox $m$ and $p$ is pending in $e$ (if some of the packets occur more than once in the sequence, then by the same lemma we may assume that there are multiple copies of those packets).
%
%We further extend the run with a reset event for middlebox $m$. Finally, we extend the scenario such that in the next $\ell$ steps $m$ will process $p_1,\dots,p_\ell$ reaching state $\sigma_m$.
%\end{proof}

The sticky states property ensures that ignoring the correlation between the state of a middlebox $m$ and the channels connected to it does not incur any precision loss w.r.t. safety.
This implies that one can also ignore correlations between the states of different middleboxes, making the network-level Cartesian abstraction defined in \secref{abs-int} precise.

%Intuitively, \lemref{sticky-packets} and \lemref{sticky-states} follow from the fact that all middleboxes can revert to their initial state and the unordered semantics enables a scenario where the particular state and packets are reconstructed.

The sticky properties formulated above are oblivious of the middlebox semantics. For the case of the packet state representation of the middlebox semantics, an even finer variant of the sticky states property of reverting unordered networks arises, which implies precision of the middlebox-level Cartesian abstraction defined in \secref{abs-int}:
%The proof of \thmref{completeness-packets} relies on a finer variant of the sticky states property of reverting unordered networks for the case of packet state representation, which we state next.
\begin{lemma} [Sticky Packet States Property]
\label{lem:sticky-packet-states}
For every channel $e$, packets $p, \tilde{p}$, middlebox $m$ and packet state $\tilde{v}$ of $\tilde{p}$ in $m$:
If, in some reachable configuration, channel $e$ contains $p$ and in some (possibly other) reachable configuration the packet state of $\tilde{p}$ in $m$ is $\tilde{v}$, then %every run can be extended such that eventually we get to a
there exists a reachable configuration where simultaneously $e$ contains $p$ and the packet state of $\tilde{p}$ in $m$ is $\tilde{v}$.
%If in some scenario channel $c$ contains $p$ and $m$ is in state $q_m$, then every scenario can be extended such that eventually we get to a configuration where simultaneously $c$ contains $p$ and $m$ is in state $q_m$.
\end{lemma}
%Intuitively, the proof of the lemma follows as all middleboxes can revert and the unordered semantics enables a scenario where the particular state and packets are reconstructed.
\iflong
\begin{proof}
Follows directly from \lemref{sticky-states} and from the bisimulation between the relation state space and the packet state space of middleboxes.
\end{proof}
\fi

Intuitively, \lemref{sticky-packets}, \lemref{sticky-states} and \lemref{sticky-packet-states} follow from the fact that all middleboxes can revert to their initial state and the unordered semantics enables a scenario where the particular state and packets are reconstructed.

\ignore{

\subsubsection{Undecidability of Safety of Reverting Networks Over Ordered Channels}
\label{sec:ordered-undecidability}
\TODO{where should this be?}

We show that if the network channels are FIFO, then we can simulate the behavior of a non-reverting network with a reverting network.
As the isolation problem for the former problem is known to be undecidable~\cite{velner2016some}, we conclude undecidability for the latter.

Intuitively our reduction makes sure that whenever one middlebox reverts the entire network reverts, i.e., all the middleboxes and all the pending packets in the channel also revert.

For this purpose we add an auxiliary \emph{wake-up} packet types and auxiliary \emph{wake-up} states for every middlebox.
Every middlebox initial state is a wake-up state, and in this state the middlebox only forwards wake-up packets and ignores (discard without any state change) other packet types.
When it forwards the wake-up packet it changes the packet type so it will also denotes the fact that the specific middlebox is in a wake-up state.
The middlebox exits the wake-up states only after it gets confirmations that all the other middleboxes in the network are in a wake-up state.

We observe that since the network is FIFO it must be the case that there are no non-wake-up packets in the channels between the middleboxes.
After it leaves the wake-up states it goes to the original initial state of the middlebox in the non-reverting network.

In this reduction, the reverting property does not change the reachability of error states, hence we get the following theorem:

\begin{theorem}
The safety verification problem over reverting FIFO networks is undecidable.
\end{theorem}

\subsubsection{Isolation for Reverting Networks with Arbitrary Number of Queries is coNP-hard}
\TODO{move somewhere. Not sure where. But needs to be after we define queries|| Why? we define queries in the syntax.}
\label{sec:conphardness}
We prove that if the number of queries in a middlebox is not fixed, then the isolation problem is coNP-hard even for one middlebox and one host.
The proof is by reduction from UNSAT.
Given a formula $\phi$ with $n$ variables $x_1,\dots,x_n$ we construct a network with one host and one middlebox $m$, such that $m$ has only one port.
The packet tag set is $x_1,\neg x_1, \dots, x_n, \neg x_n$, i.e., there are $2n$ packet types.
The middlebox has two nullary relations $O_i,V_i$ for every $i\in\{1,\dots,n\}$, where intuitively, $O_i$ indicates whether a packet of type $x_i$ or $\neg x_i$ already occurred and $V_i$ indicates if the value of the first such packet is true or false.
Initially all the relations are initialized to false.
The relation $V_i$ is updated only if $O_i$ is false, and then $O_i$ is also updated.
The middlebox discards all packets.
In addition, whenever the interpretation of $O_i$ and $V_i$ satisfies $\phi$ an abort state is reached.
Clearly, the size of the code of $m$ is polynomial and isolation is violated if and only if $\phi$ is satisfiable.
We note that possible resets do not affect the isolation property.
\begin{theorem}
The isolation problem for reverting unordered networks is coNP-hard.\footnote{The safety verification
problem and the isolation problem are equivalent.}
\end{theorem}


}


\subsection{Summary of the Different Semantics and their Relations}
We have defined four variants of the network transitions over concrete ordered configurations, where both
\[
\begin{array}{ccc}
{\BB{\Net}^{o}} \subseteq {\BB{\Net}^{u}} \subseteq {\BB{\Net}^{ur}}
&
\text{ and }
&
{\BB{\Net}^{o}} \subseteq {\BB{\Net}^{or}} \subseteq {\BB{\Net}^{ur}}
\end{array}
\]
hold ($o$ stands for ``ordered'', $u$ stands for ``unordered'' and $r$ stands for ``reverting''.)

By plugging-in the two representations of middleboxes in the definition of the network semantics, we obtain two variants of the network semantics for each of the four variants considered so far.
In the sequel, we use a $pa$ subscript to refer to the packet effect semantics, and no subscript to refer to the relation effect semantics.
%packet state network semantics.
%
The bisimulation between middlebox representations is lifted to a bisimulation between each relation state network semantics and the corresponding packet state network semantics.
Therefore, the following holds:
%We use \TODO{notation} to denote them.
%Next, we perform abstract interpretation on the packet state representation of networks.

\begin{lemma}
For every semantic identifier $i \in \{o,u,or,ur\}$, $\err \in {\BB{\Net}^{i}}$ if and only if $\err \in {\BBsub{\Net}{pa}^{i}}$.
\end{lemma}

\ignore{
\TODO{SH: revise}
\para{Packet State Network Configurations}
The packet state network configurations are defined as $(\sigma, \pi) \in \PState = (M\to \PState[M])\times(E \to \packets^{*})$, where
$\PState[M] = \bigcup\limits_{m\in M}\PState[m]$ denotes the
set of middlebox states in the packet state representation of all middleboxes in the network.
Error configurations, denoted $\err$, are defined as in \defref{error-conf}.

\para{Initial Configuration}
The initial packet state configuration is $(\PState(\sigma_I),\lambda\,e\in E\,.\, \epsilon)$.

\para{Packet State Network Transitions}
The four semantics of network transitions presented in \secref{network-semantics} are naturally adapted to packet state configurations, the only difference is that the middlebox state transitions are over the packet space, as described in \secref{packet-space-concrete-transformer}. The collecting semantics are also adapted. Of special interest are the collecting packet state ordered semantics, denoted ${\BBsub{\Net}{pa}^{o}}$, and the collecting packet state unordered reverting semantics, denoted ${\BBsub{\Net}{pa}^{ur}}$. %\TODO{fix semantics notation}

%Of special interest are the packet state ordered transitions, denoted $\xRightarrow{}_o$, and the packet state unordered reverting transitions, denoted $\xRightarrow{}_{ur}$.

%We denote the collecting packet state ordered semantics by $\BB{\Net}{o}{pa}$ and the collecting packet state unordered reverting semantics by $\BB{\Net}{ur}{pa}$.

The bisimulation between middlebox representations can be lifted to a bisimulation between each relation state network semantics and the corresponding packet state network semantics.
Therefore, the following holds:
%We use \TODO{notation} to denote them.
%Next, we perform abstract interpretation on the packet state representation of networks.

\begin{lemma}
For every semantic identifier $i \in \{o,u,or,ur\}$, $\err \in {\BB{\Net}^{i}}$ if and only if $\err \in {\BBsub{\Net}{pa}^{i}}$.
\end{lemma}

}


==> running_example.tex <==
\section{Running example}\label{sec:running_example}
\TODO{Needs cleanup, and to be moved elsewhere.}

Consider the network illustrated in Figure~\ref{fig:run_example}.
The network consists of two internal hosts $h_0, h_1$ that reside on port $0$ and two external hosts $h_2, h_3$ that reside on port $1$.
$h_3$ is a malicious hosts for the internal hosts and their network administrator prevents them from sending it any packets.
The internal and external hosts are connected with a hole-punching firewall that prevents untrusted hosts to send packets to the internal hosts.
An external host becomes trusted only after an internal host sends it a packet.
In addition, the firewall has the safety property that a malicious host is never trusted (see code in Figure~\ref{fig:example_code}).
The state set of the firewall is the state set of the $\mathit{trusted}$ relation, i.e., which hosts are in the relation.
The set of abstract states could only keep track on whether each host was ever in the relation and whether it was ever not in the relation.
We implement the fixed point algorithm with a Datalog program (illustrated in Figure~\ref{fig:example_data_code}).
In order to allow using the negation of a property (i.e., to specify that a host is not malicious), we increase the arity of the predicate such that it will include also a Boolean that indicates whether the property holds or not.
For example,``host $h$ is not malicious" is encoded as $\mathit{malicious}(h,0)$.
The Datalog code has two parts.
The first part describes the initial values of the relation and the topology of the network and it is independent of the middlebox code.
For example, the code $\mathit{NeighborHostPackets}_0(s,d,t) :- s=0, \mathit{malicious}(d,0)$ describes the fact that the network administrator prevents host $h_0$ from sending packets to the malicious host.
The second part describes the functionality of the middlebox.
For example, the code $\mathit{trusted}(d,1) :- \mathit{packetSeen}_0(s,d,t)$ corresponds to the fact that a host becomes trusted only if it is the destination of a packet that an internal host sent.
We use the generated Datalog program to query whether the nullary predicate $\mathit{abort}$ is true in the least fixed point.
The network is safe if and only if at the fixed point its value is false.

\TODO{The algorithm is not accurately depicted - we don't have a Datalog relation for every middlebox relation, we have a packet state Datalog relation.}

\begin{figure}
\begin{center}
\includegraphics[width=0.3\textwidth]{img/running-example}
\end{center}
\caption{Example network}\label{fig:run_example}
\end{figure}

\begin{figure}
\begin{center}
\begin{lstlisting}[language=Python,basicstyle=\small]
FW(s,d,t,p)
  requires not (malicious(s) and
                trusted(s))

  when p=0
    update trusted(d) = true
    output {(s,d,t,1)}
  when p=1 and trusted(s)
    output {(s,d,t,0)}
\end{lstlisting}
\end{center}
\caption{Example firewall code}\label{fig:example_code}
\end{figure}

\begin{figure}
\begin{center}
\begin{lstlisting}[language=Prolog,basicstyle=\small]

%%% initialization

malicious(s,1) :- s=3
malicious(s,0) :- s!=3

NeighborHostPackets_0(s,d,t) :- s=0, malicious(d,0)
NeighborHostPackets_0(s,d,t) :- s=1, malicious(d,0)

NeighborHostPackets_1(s,d,t) :- s=2
NeighborHostPackets_1(s,d,t) :- s=3


packetSeen_0(s,d,t) :- NeighborHostPackets_0(s,d,t)
packetSeen_1(s,d,t) :- NeighborHostPackets_1(s,d,t)


%%% program

abort :- malicious(s,1), trusted(s,1)
trusted(d,1) :- packetSeen_0(s,d,t)
packetSent_0(s,d,t) :- packetSeen_1(s,d,t), trusted(s,1)
packetSent_1(s,d,t) :- packetSeen_0(s,d,t)
\end{lstlisting}
\end{center}
\caption{Example Datalog code}\label{fig:example_data_code}
\end{figure}


==> sticky-semantics.tex <==
\section{Sticky Network Semantics}
\label{sec:sticky-semantics}

\TODO{RM: consider dropping the vector notation as it doesn't seem to be
used.}

\para{Motivation}
Recall that concrete unordered configurations are defined as $\Sigma^u = (M\to \Sigma^r[M])\times(E \to \mset{P})$.
%
To simplify the presentation, we will use a vector representation.
Let $m_1,\ldots,m_\ell$ be an enumeration of $M$ and $e_1,\ldots,e_k$ be an enumeration of $E$.
%
Recall that $\Sigma^r[m]$ denotes the set of middlebox states of $m\in M$.
Let $\Sigma^r[e] : \mset{P}$ denote the set of states (i.e., content)
of a channel $e$.
%
Unordered configurations can be therefore represented by the set of vectors
$\Sigma^r[m_1]\times\ldots\times\Sigma^r[m_{\ell}]\times \Sigma^r[e_1]\times\ldots\times \Sigma^r[e_k]$.
%
The state space of the network is therefore $\pset(\Sigma^r[m_1]\times\ldots\times\Sigma^r[m_{\ell}]\times \Sigma^r[e_1]\times\ldots\times \Sigma^r[e_k])$. An explicit search for a state violating the safety property would be exponential in the state space (and thus doubly-exponential in the number of hosts in the network).

\subsection{Sticky Properties}

However, reverting networks have two useful properties that can help us reduce the complexity of searching for a violating state, namely the \emph{sticky states} property and the \emph{sticky packets} property. Intuitively, the sticky properties state that if an event occurs in some run of the network, then any run has an extension in which that event occurs. Consequently, we can disregard the multiplicity of packets on the channels and the correlation between the state of a middlebox $m$ and the states of other middleboxes as well as the states of the channels that are not connected to the middlebox $m$.

The following lemma shows that reverting networks have the sticky packet property.

\begin{lemma}
\label{lem:sticky_packets}
For every channel $c$ and packet $p$:
If in some scenario $c$ contains $p$, then every scenario can be extended such that $c$ will eventually contain $p$.

Moreover, every scenario can be extended such that $c$ will eventually contain $n$ copies of $p$ (for every $n>0$).
\end{lemma}
\begin{proof}
The proof relies on the reverting property and on the fact that the channels are unordered.

Let $s_0$ be a scenario in which $p$ occurs in $c$.
Consider an arbitrary scenario $s$. One can extend $s$ with the following scenario:
First all the middleboxes in $s$ return to their initial state.
Second, scenario $s_0$ occur, i.e., only packets from scenario $s_0$ are processed, and the other packets are ignored.
This extension is possible because the channels are unordered.

To construct a scenario in which $c$ contains $n$ copies of $p$, we just concatenate the above mentioned extension $n$ time.
\end{proof}

We now show that reverting networks have the sticky states property.

\begin{lemma}
\label{lem:sticky}
For every channel $c$ a packet $p$, a middlebox $m$ and a state $q_m$:
If in some scenario channel $c$ contains $p$ and $m$ is in state $q_m$, then every scenario can be extended such that eventually we get to a configuration where simultaneously $c$ contains $p$ and $m$ is in state $q_m$.
\end{lemma}
\begin{proof}
Let $(p_1,\dots,p_\ell)$ be the sequence of packets that $m$ processed from the latest reset until it arrives to state $q_m$ in the given witness scenario.

Consider an arbitrary scenario.
By Lemma~\ref{lem:sticky_packets} we can extend this scenario such that $p_1,\dots,p_\ell$ are pending packets in the ingress channel of middlebox $m$ and $p$ is pending in $c$ (if some of the packets occur more than once in the sequence, then by the same lemma we may assume that there are multiple copies of those packets).

We further extend the scenario with a reset event for middlebox $m$. Finally, we extend the scenario such that in the next $\ell$ steps $m$ will process $p_1,\dots,p_\ell$ reaching state $q_m$.
\end{proof}

\subsection{Formal Semantics}

\para{Sticky Channels Network Configurations}

When a network has the sticky packets property, it is no longer necessary to maintain the cardinality of every packet type on every channel. Instead, it is sufficient to record whether a packet arrived on the channel at some point.
%
We can then define the \emph{sticky channel configuration} of a network as $\Sigma^s = (M\to \Sigma^r[M])\times(E \to 2^P)$. Which assigns communication channels to sets of packets, abstracting away the cardinality of each packet.

\para{Sticky Channels Network Transitions}
We define the sticky Channels semantics of a transition in the network as $(\sigma,C) \xrightarrow{p,e,m}_s (\sigma',C')$ where
the following hold:
(i) $p$ is some packet on the channel $e \in E$,
(ii) the channel $e$ is an ingress channel of middlebox $m$,
(iii) there exists a command $c$ in middlebox $m$ s.t. $\sembr{c}_{pre}$ holds in state $\sigma(m)$ for packet $p$,
(iv) the safety condition $\msafe{m}$ of the middlebox $m$ holds for the middlebox state $\sigma(m)$ for packet $p$,
(v) $C'$ is the result of adding the result of $\sembr{c}_{out}$ to the the appropriate channels via set union, and
(vi) $\sigma'$ is either the result of updating $\sigma(m)$ with $\sembr{c}_{upd}$ or it is the state
$\sigma_I(m)$ where the middlebox $m$ is in its initial state---the state of all other middleboxes equals their state in $\sigma$.


